Learning Mixtures of Graphs from Epidemic Cascades

We consider the problem of learning the weighted edges of a balanced mixture of two undirected graphs from epidemic cascades. While mixture models are popular modeling tools, algorithmic development with rigorous guarantees has lagged. Graph mixtures are apparently no exception: until now, very little is known about whether this problem is solvable. To the best of our knowledge, we establish the first necessary and sufficient conditions for this problem to be solvable in polynomial time on edge-separated graphs. When the conditions are met, i.e., when the graphs are connected with at least three edges, we give an efficient algorithm for learning the weights of both graphs with optimal sample complexity (up to log factors). We give complimentary results and provide sample-optimal (up to log factors) algorithms for mixtures of directed graphs of out-degree at least three, for mixture of undirected graphs of unbalanced and/or unknown priors.

==> files/alpha_new-v3.tex <==
In the context of unknown priors, we first learn alpha, then recover the weights through an adaptation of Claim \ref{claim:eststar} and Claim \ref{claim:estline} for unbalanced mixtures.  The proof can be found in Supplemental materials \ref{app:unknownAlpha}.

\begin{theorem}
	Under Assumptions \ref{ass:main}, in the limit of infinite samples, we can recover the unknown priors of the mixture, as well as all the weights of the edges for any connected graph on five nodes or more. If the graph has four nodes, it is still achievable if there exists a star vertex.
\end{theorem}


==> files/gengraph-v4.tex <==
In this section, we provide our main algorithm that recovers the edge weights on the graph under the conditions presented in Theorem \ref{thm:mainnotexist}. We focus on the setting of balanced mixture priors for ease of exposition. We refer the reader to Supplementary \ref{app:unknownAlpha} for the results on the unbalanced mixture case. 



\paragraph{Outline of Main Algorithm~\ref{algo:generalGraph}}
{\color{blue} Edited the whole subsection below.}
We first learn whether an edge $(u,v)$ exists in $E_1 \cup E_2$ using a simple estimator (Section \ref{sec:struct}). This also provides us with the degree of each node with respect to $E_1 \cup E_2$.

We show if a node is of degree at least three (e.g. node $u$ in Figure~\ref{fig:star}), there exists an estimator that uses the {\em star structure} to learn all the edges (i.e. the weights of the two mixtures for these edges) adjacent to this node {\em independently} of the rest of the graph. Otherwise, if a node is of degree two (e.g. node $u$ in Figure~\ref{fig:line}) we design a different estimator which leverage a {\em line structure} to learn all the edges adjacent to this node {\em independently}. We present the above estimators for an balanced mixtures in  (Section \ref{sec:estimators}). We require Condition~\ref{ass:main} for the existence of the proposed estimators.

Our main algorithm (Algorithm \ref{algo:generalGraph}), maintains a set of {\em learned nodes}. A node is a  {\em learned node} is the weights for all the edges adjacent to it is learned. The algorithm begins with learning two connected nodes (two nodes having an edge in between). Next it proceeds iteratively, by learning the weights of the edges connected to one {\em unlearned neighbor} of the {\em learned nodes}. The algorithm terminates, when all the nodes in $V$ are learned.  In Theorem~\ref{thm:mainnotexist}, we show that under Conditions \ref{ass:necessary}, it is possible to iteratively learn all the nodes in $V$ using the proposed estimators. 

\textbf{Biased mixture:} We require different estimators for the known but general $\alpha$ case, which are deferred to Supplementary \ref{app:unknownAlpha}. We note that Algorithm \ref{algo:generalGraph} works for general $\alpha$ as well with the appropriate estimators.

\subsection{Learning the Edges in $E_1 \cup E_2$}\label{sec:struct}
We recall that $I^m_0$ is the set containing the unique source of the epidemic for cascade $m$.

\begin{definition} 
Let $u$ and $a$ be two distinct nodes of V. We define:
$$\hat{X}_{ua} := \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \rightarrow a, u \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \in I_0^m}} \to_{M \to \infty} X_{ua}.$$
\end{definition}

We compute the limit of this estimator:

\begin{claim} \label{cl:trivialXab}
If $u$ and $a$ are two distinct nodes of $V$ such that $(u,a) \in E_1 \cup E_2$, then: 
$$X_{ua} =  \Pr(u \rightarrow a ~|~ u \in I_0) =  \frac{p_{ua} + q_{ua}}{2} \geq \frac{p_{min}}{2}.$$
\end{claim}
\begin{proof}
Using the law of large number and Slutsky's Lemma, it is immediate to see that $X_{ua} = \Pr(u \rightarrow a ~|~ u \in I_0)$. Then:
%  \begin{align*}
%      X_{ua}  &= \frac{\Pr(u \rightarrow a, ~ u \in I_0~|~L^m=1)\Pr(L^m=1) + \Pr(u \rightarrow a, ~ u \in I_0~|~L^m=2)\Pr(L^m=2)}{\Pr(u \in I_0~|~L^m=1)\Pr(L^m=1) + \Pr(u \in I_0~|~L^m=2)\Pr(L^m=2)} \\
%     &= \frac{p_{ua} \frac{1}{N}\frac{1}{2} + q_{ua} \frac{1}{N}\frac{1}{2} }{\frac{1}{N}\frac{1}{2} + \frac{1}{N}\frac{1}{2}} = \frac{p_{ua} + q_{ua}}{2}.
% \end{align*}
 \begin{align*}
     X_{ua} &= \Pr(u \rightarrow a, L_m = 1 ~|~ u \in I_0)\\
     &\quad + \Pr(u \rightarrow a, L^m=2~| ~ u \in I_0) \\
     &= \Pr(L_m = 1 ~|~ u \in I_0)\Pr(u \rightarrow a ~|~ u \in I_0, L_m = 1) \\
     &\quad + \Pr(L_m = 2 ~|~ u \in I_0)\Pr(u \rightarrow a ~|~ u \in I_0, L_m = 2)\\
    &= \frac{1}{2} \cdot p_{ua} + \frac{1}{2} \cdot q_{ua}
\end{align*}
\end{proof}

This estimator can therefore be used to learn whether or not there exists an edge in the mixture.
\begin{corollary}
	Let $u$ and $a$ be two distinct nodes of $V$. Then:\\
	1. If there exists an edge between $u$ and $a$ in $E_1 \cup E_2$, then $X_{ua} \geq \frac{p_{min}}{2} > 0$.\\
	2.If there exists no edge between $u$ and $a$, then $X_{ua} = 0$.
\end{corollary}

%We turn this corollary into an algorithm:
\begin{corollary}\label{corollary:LearnEdges}
	We can write an algorithm \textsc{LearnEdges}, which takes as inputs all the $X_{ua}$ for all pairs $(u,a)$, and returns all the edges of $E_1 \cup E_2$ (See Supplemental Materials, Algorithm \ref{app:learnEdges}).
\end{corollary}

\subsection{Learning Star and Line Vertices: Base Estimators} \label{sec:estimators}
In this section, we show how we recover the weights of both mixture components in a node-by-node fashion. We start from the easy case, when the node we consider has degree at least three.

\subsubsection{Star vertex}
\begin{figure}
\centering
\begin{tikzpicture}
    \node[main node, fill=white] (0) {$a$};
    \node[main node, fill=pink] (1) [right = 0.5cm of 0] {$u$};
    \node[main node, fill=white] (2) [above right = 0.5cm and 0.2cm of 1]  {$b$};
    \node[main node, fill=white] (3) [below right = 0.5cm and 0.2cm of 1] {$c$};

    \path[draw,thick]
    (0) edge node {} (1)
    (1) edge node {} (2)
    (1) edge node {} (3);
\end{tikzpicture}
\caption{A star vertex $u$, with edges $(u,a), (u,b)$ \\and $(u,c)$ in $E_1 \cup E_2$.}\label{fig:star}
\end{figure}
\begin{figure}
\centering
\begin{tikzpicture}
    \node[main node, fill=white] (0) {$a$};
    \node[main node, fill=pink] (1) [right = 0.5cm of 0] {$u$};
    \node[main node, fill=white] (2) [right = 0.5cm of 1]  {$b$};
    \node[main node, fill=white] (3) [right = 0.5cm of 2] {$c$};
    \path[draw,thick]
    (0) edge node {} (1)
    (1) edge node {} (2)
    (2) edge node {} (3);
\end{tikzpicture}
% \includegraphics[width=0.4\linewidth]{line.jpg}
% \caption{line}\label{fig:line}
\caption{A line vertex $u$, with edges $(u,a), (u,b)$ and $(b,c)$ in $E_1 \cup E_2$.}\label{fig:line}
\end{figure}
% \includegraphics[width=0.3\linewidth]{star.jpg}
%\caption{Left: A vertex $u$ of degree $\ge 3$ with any of its three distinct neighbors. Right: A line $a-u-b-c$ rooted at vertex $u$ of degree 2.}\label{fig:star}
% \begin{definition}
% Let $i, j, k$ and $l$ be four distinct nodes of V, such that $(i,j), (i,k)$ and $(i,l)$ belong in $E_1 \cup E_2$. We call such four nodes a \textbf{star structure rooted in $i$} (see Figure \ref{fig:star}). For such a structure, define:
% {\color{orange} Might want to make $j$ the central node to be more coherent with the line structure.}
% \begin{enumerate}
%     \item For $r\neq s \in \{j,k,l\},~Y_{ur, is} = \Pr(i \rightarrow r, i \rightarrow s ~|~ i \in I_0)$
%     \item $Z_{ua, ub, uc} = \Pr(i \rightarrow j, i \rightarrow k, i \rightarrow b~|~ i \in I_0)$
% \end{enumerate}    
% \end{definition}
\begin{definition}
A \underline{star vertex} is a vertex $u \in V$ of degree at least three in $E_1 \cup E_2$. Let $a$ and $b$ be two distinct neighbors of $u$. For a star vertex, we define:
$$\hat{Y}_{ua, ub} =  \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \rightarrow a, u \rightarrow a, u \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \in I_0^m}} \to_{M \to \infty} Y_{ua, ub}.$$
\end{definition}
\begin{claim}\label{claim:eststar}
In the limit of infinite samples, for $u$ star vertex and $a$, $b$ and $c$ as in Figure \ref{fig:star}:
 $$Y_{ua, ub} = \Pr(u \rightarrow a, u \rightarrow b ~|~ u \in I_0) = \frac{p_{ua}p_{ub} + q_{ua}q_{ub}}{2}.$$
\end{claim}
\begin{proof}
	One crucial point to notice is that if $u$ is the source, no other node could have infected $a$ or $b$ before $u$ infected them. Therefore, we know for a fact that both $a$ and $b$ are susceptible. If the source had been any other node, the probability that $a$ (or $b$) was not removed would have depended on the (unknown) weights of both mixtures, and we could not have obtained the simplification desired.
	Once this has been noticed, the proof for $Y_{ua, ub}$ is almost identical to the proof in Claim \ref{cl:trivialXab}. 
\end{proof}


\begin{lemma}\label{lem:star}
Suppose Conditions \ref{ass:necessary} and  \ref{ass:main} are verified. Let $s_{ua} \in \{-1,1\}$. In the setting of infinite samples, the weight of any edge $(u,a)$ connected to a star vertex $u$, with distinct neighbors $a$, $b$ and $c$ in $E_1 \cup E_2$, is given by:
\begin{align*}
p_{ua} &= X_{ua} + s_{ua} \sqrt{\frac{(Y_{ua,ub} - X_{ua}X_{ub})(Y_{ua,uc} - X_{ua}X_{uc})}{Y_{ub,uc} - X_{ub}X_{uc}}},\\ 
q_{ua} &= X_{ua} - s_{ua} \sqrt{\frac{(Y_{ua,ub} - X_{ua}X_{ub})(Y_{ua,uc} - X_{ua}X_{uc})}{Y_{ub,uc} - X_{ub}X_{uc}}}.
\end{align*} 
\end{lemma}
\begin{proof}
We notice that for $i \neq j \in \{a,b,c\}$, $Y_{ui, uj} - X_{ui}X_{uj} = \frac{(p_{ui} - q_{ui})(p_{uj} - q_{uj})}{4}$. Therefore,
%\begin{align*}
%    Y_{ui, uj} - X_{ui}X_{uj} %&= \frac{p_{ui}p_{uj} + q_{ui}q_{uj}}{2} -\left( \frac{p_{ui} + q_{ui}}{2}\right)\left( \frac{p_{uj} + q_{uj}}{2}\right) \\
%    %&= \frac{1}{4}(p_{ui}p_{uj} - p_{ui}q_{uj} + q_{ui}q_{uj} - q_{ui}p_{uj}) \\
%    &= \frac{(p_{ui} - q_{ui})(p_{uj} - q_{uj})}{4}.
%\end{align*}

\begin{align*}
&\sqrt{\frac{(Y_{ua,ub} - X_{ua}X_{ub})(Y_{ua,uc} - X_{ua}X_{uc})}{Y_{ub,uc} - X_{ub}X_{uc}}}\\
&= \sqrt{\frac{\frac{(p_{ua} -  q_{ua})(p_{ub} - q_{ub})}{4} \cdot \frac{(p_{ua} -  q_{ua})(p_{uc} - q_{uc})}{4}}{\frac{(p_{ub} -  q_{ub})(p_{uc} - q_{uc})}{4}}} \\
   &= \frac{|p_{ua} - q_{ua}|}{2}.
\end{align*}
Since $X_{ua} = \frac{p_{ua} + q_{ua}}{2}$, we have $p_{ua} = \frac{p_{ua} + q_{ua}}{2} +  \frac{|p_{ua} - q_{ua}|}{2}$ or $p_{ua} = \frac{p_{ua} + q_{ua}}{2} -  \frac{|p_{ua} - q_{ua}|}{2}$, which gives the required result.
\end{proof}

\begin{corollary}\label{corollary:LearnStar}
	We can write an algorithm \textsc{LearnStar}, which takes as input a star vertex $u$, the set of edges of $E_1 \cup E_2$, and all the $X_{ui}$ and $Y_{ui,uj}$ for all $(i,j)$ distinct neighbors of $u$, and returns all the weights of the edges connected to $u$ in both mixtures (See Supplemental Materials, Algorithm \ref{app:learnStar}).
\end{corollary}

\subsubsection{Line vertex}
\begin{definition}
Let $u, a, b$ and $c$ be four distinct nodes of V, such that $(a,u), (u,b)$ and $(b,c)$ belong in $E_1 \cup E_2$. Suppose also that $u$ has degree exactly two in $E_1 \cup E_2$. We call such a node $u$ a \underline{line vertex} (see Figure \ref{fig:line}). For a line vertex, we define:
% {\color{orange} I need to fix the sign by adding some $sgn(Y -XX)$ factors around.}
\begin{enumerate}
	\item $\hat{Y}^|_{ua, ub} =  \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \rightarrow a, u \rightarrow a, u \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \in I_0^m}} \to_{M \to \infty} Y^|_{ua, ub}.$
	\item $\hat{Y}^|_{ub,bc} =  \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \rightarrow b, b \rightarrow c, u \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \in I_0^m}} \to_{M \to \infty} Y^|_{ub, bc}.$
	\item $\hat{Z}^|_{ua, ub, bc} =  \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \rightarrow a, u \rightarrow b, b \rightarrow c, u \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \in I_0^m}} \to_{M \to \infty} Z^|_{ua, ub, bc}.$
\end{enumerate}    
\end{definition}

\begin{claim}\label{claim:estline}
In the limit of infinite samples, for $u$ line vertex and $a$, $b$ and $c$ as in Figure \ref{fig:line}:
\begin{enumerate}
    \item $Y^|_{ua,ub} = Pr(u \rightarrow a, u \rightarrow b ~|~ u \in I_0) = \frac{p_{ua}p_{ub} + q_{ua}q_{ub}}{2}$
    \item $Y^|_{ub,bc} = \Pr(u \rightarrow b, b \rightarrow c ~|~ u \in I_0) = \frac{p_{ub}p_{bc} + q_{ub}q_{bc}}{2}$.
    \item $Z^|_{ua,ub,bc} = \Pr(u \rightarrow a, u \rightarrow b, b \rightarrow c~|~ u \in I_0) = \frac{p_{ua}p_{ub}p_{bc} + q_{ua}q_{ub}q_{bc}}{2}$.
\end{enumerate}
\end{claim}
\begin{proof}
The result for $Y^|_{ua,ub}$ was proven in Claim \ref{claim:eststar}. 

However, the proof for $Y^|_{ub,bc}$ and $Z^|_{ub,bc,bc}$ is different. The proof relies heavily on the fact that $u$ is of degree 2, which implies in particular that there are no edges between $u$ and $c$ (or in other words, $p_{uc} = q_{uc} = 0)$.
\begin{align*}
    Y^|_{ub,bc} &= \Pr(u \rightarrow b, b \rightarrow c ~|~ u \in I_0) \\
    & = \Pr(u \rightarrow b, u \not \rightarrow c, b \rightarrow c ~|~ u \in I_0) \\
    &= \frac{p_{ub}(1-p_{uc})p_{bc}\frac{1}{N}\frac{1}{2} + q_{ub}(1-q_{uc})q_{bc} \frac{1}{N}\frac{1}{2} }{\frac{1}{N}\frac{1}{2} + \frac{1}{N}\frac{1}{2}}\\
    &= \frac{p_{ub}p_{bc} + q_{ub}q_{bc}}{2}.
\end{align*}
The proof is almost identical for $Z^|_{ub,bc,bc}$.
\end{proof}

\begin{lemma}\label{lem:line}
Suppose Conditions \ref{ass:necessary} and  \ref{ass:main} are verified. Let $s_{ua}, s_{ub}$ and $s_{bc}$ be in $\{-1,1\}$, and let $R^| = X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}$. In the setting of infinite samples, the weights of the edges for a line structure are then given by: 
%{\color{red} I removed the others as we need only this edge for the proof! Guess I was wrong, we need them all!}
\begin{align*}
    p_{ua} &= X_{ua} + s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub})R^| }{Y^|_{ub, bc} - X_{ua}X_{bc}}},\\
    q_{ua} &= X_{ua} - s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub})R^| }{Y^|_{ub, bc} - X_{ua}X_{bc}}}, \\
    p_{bc} &= X_{uc} + s_{bc} \sqrt{\frac{(Y^|_{ub, bc} - X_{ua}X_{bc})R^| }{Y^|_{ua,ub} - X_{uc}X_{ua}}},\\
    q_{bc} &= X_{uc} - s_{bc} \sqrt{\frac{(Y^|_{ub, bc} - X_{ua}X_{bc})R^| }{Y^|_{ua,ub} - X_{uc}X_{ua}}}\\
    p_{ub} &= X_{ub} + s_{ub} \sqrt{\frac{(Y^|_{uc,ua} - X_{uc}X_{ua})(Y^|_{ub, bc} - X_{ua}X_{bc})}{R^|}}, \\
    q_{ub} &= X_{ub} - s_{ub} \sqrt{\frac{(Y^|_{uc,ua} - X_{uc}X_{ua})(Y^|_{ub, bc} - X_{ua}X_{bc})}{R^|}}. \\
\end{align*}
\end{lemma}
\begin{proof} 
In this case, there is no edge between $u$ and $c$, which implies that $p_{uc} = q_{uc} = 0$.  Hence, we cannot use a variation of the equation above for finding the edges of a star structure without dividing by zero. Therefore, we need to make use of the estimator $Z^|_{ua, ub, bc}$. We notice a remarkable simplification:
\begin{align*}
&X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}\\
&= \frac{1}{4}(p_{ua} - q_{ua})(p_{bc} - q_{bc}).
\end{align*}

We  then use the same proof techniques as in Lemma \ref{lem:star}, and obtain the required result. See detailed calculations in Supplemental materials \ref{app:line}.
\end{proof}

\begin{corollary}\label{corollary:LearnLine}
	We can write an algorithm \textsc{LearnLine}, which takes as input a line vertex $u$, the set of the edges of $E_1 \cup E_2$, and the limit of the estimators $X_{ua}$, $X_{ub}$, $X_{bc}$,  $Y^|_{ua, ub}$, $Y^|_{ub, bc}$, $Z^|_{ua, ub, bc}$ for $a$, $b$ and $c$ as in Figure \ref{fig:line}, and returns the weights of the edges $(u,a), (u,b)$ and $(b,c)$ in both mixtures (see Supplementary Materials, Algorithm \ref{app:learnLine}).
\end{corollary}


\subsection{Resolving Sign Ambiguity across Base Estimators}
The following lemma handles the sign ambiguity ($s_{ua}$) introduced above.
\begin{lemma}\label{lem:sign}
Suppose Condition \ref{ass:necessary} and \ref{ass:main} are true, in the setting of infinite samples, for edges $(u,a), (u,b)$ with $a\ne b$ for any vertex $u$ with degree $\ge 2$, the sign pattern $s_{ua}, s_{ub}$ satisfy the following relation.
\[
s_{ua}s_{ub} = \mathsf{sgn}(Y_{ua,ub} - X_{ua}X_{ub}).
\]
\end{lemma}
\begin{proof}
From previous analysis, we have $\mathsf{sgn}(p_{ua} - q_{ua}) = s_{ua}$. Therefore:
\begin{align*}
\mathsf{sgn}(Y_{ua,ub} - X_{ua}X_{ub}) &= \mathsf{sgn}\left(\frac{(p_{ua} - q_{ua})(p_{ub} - q_{ub})}{4}\right) \\
&=  s_{ua}s_{ub}.
\end{align*}
\end{proof}
Thus fixing sign of one edge gives us the signs of all the other edges adjacent to a star vertex. A similar relationship can be established among the edges of a line vertex, using $ \mathsf{sgn}\left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}\right) $.

\subsection{Main Algorithm}
We can now turn to the main algorithm (see Algorithm \ref{algo:generalGraph}). This algorithm first uses the algorithms \textsc{LearnEdges} (Corollary \ref{corollary:LearnEdges}) to learn all the edges of $E_1 \cup E_2$.  It then calls \textsc{Learn2Nodes} as an initialization, which learns all weights of the edges connected to two initial nodes (see Supplemental Materials, Algorithm \ref{app:learn2Nodes}). The set $S$, which only contains nodes for which the weights of each incident edge has been learned, is initialized with these two nodes. 

Then, at each iteration, of our algorithm we pick one node connected to $S$. If this node is a star vertex, we learn all the weights of its neighborhood using    \textsc{LearnStar} (Corollary \ref{corollary:LearnStar}). If this node is a line vertex, we we learn all the weights of its neighborhood using \textsc{LearnLine} (Corollary \ref{corollary:LearnLine}). If this node has degree one, we have already learned all the weights of the edges connected to it, so we proceed without doing anything. Finally, since we have learned all the weights of the edges connected to this new node, we can add it to $S$. We keep growing $S$ until $S = V$.




\begin{comment}
%We will explain each procedure of the algorithm and then give a proof of correctness. 
% \begin{algorithm}[H] 
% \caption{Learn the undirected edges of any mixture of connected graphs.}\label{algo:generalGraph}
% \begin{algorithmic}[1]
% %$T^{'}$ is an $n_{nodes}$x$M$ matrix: 
% \Procedure{LearnMixtures}{$\{h_{i,S}\}_{i \in V}^{|S| \leq d}$} 
% \State\textcolor{gray}{// Initialization.}
% \State $nodes\_seen \gets \emptyset$
% \State $nodes\_to\_learn \gets \emptyset$
% \State $nodes\_left \gets V \setminus nodes\_seen$
% \State
% \State\textcolor{gray}{// Learn all the edges of the mixture among 4 initial nodes.}
% \State \textsc{Pick} 4 connected nodes $i,j,k$ and $l$
% \State $nodes\_to\_learn \gets \{i,j,k,l\}$
% \State $nodes\_left \gets nodes\_left \setminus \{i,j,k,l\}$
% \State $\textsc{Learn4Nodes}(i,j,k,l)$
% \State $nodes\_seen \gets \{i,j,k,l\}$
% \State
% \State\textcolor{gray}{// Learn the rest of the mixture, one edge at a time.}
% \While{$nodes\_to\_learn \neq \emptyset$}
% \State $current\_node = \textsc{Pop}(nodes\_to\_learn)$
% \State\textcolor{gray}{// If we can, we use the star primitive.}
% \If{$\textsc{Degree}(current\_node) \geq 3$} 
% \State $old\_neighbor =$ any node in $\textsc{Neighbor}[current\_node] \cap nodes\_seen$
% \State\textcolor{gray}{// We learn all the edges between $current\_node$ and its unseen neighbors.}
% \For{$new\_neighbor$ in $\textsc{Neighbor}[current\_node] \cap nodes\_left$}
% \State $other\_neighbor = $ any node in $\textsc{Neighbor}[current\_node] \setminus \{old\_neighbor, new\_neighbor \}$
% \State $\textsc{LearnStar}(current\_node, old\_neighbor, new\_neighbor, other\_neighbor)$
% \If{$new\_neighbor \notin nodes\_to\_learn$}
% \State $nodes\_to\_learn.add(new\_neighbor)$
% \EndIf
% \EndFor
% \Else\textcolor{gray}{ // If we cannot use the star primitive, we use the line primitive.}
% \If{$\textsc{Neighbor}[current\_node] \cap nodes\_left \neq \emptyset$}
% \State $new\_neighbor \gets$ only node in $\textsc{Neighbor}[current\_node] \cap nodes\_left$
% \State $old\_neighbor = $ any node in $\textsc{Neighbor}[current\_node] \cap nodes\_seen$
% \State $old\_neighbor\_of\_neighbor = $ any node in $\textsc{Neighbor}[old\_neighbor] \cap nodes\_seen$
% \State $\textsc{LearnLine}(new\_neighbor, current\_node, old\_neighbor, old\_neighbor\_of\_neighbor)$
% \If{$new\_neighbor \notin nodes\_to\_learn$}
% \State $nodes\_to\_learn.add(new\_neighbor)$
% \EndIf
% \EndIf
% \EndIf
% \State $nodes\_seen.add(current\_node)$
% \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}



% A connected set of 4 nodes induce the following 6 connected isomorphic formations.
% \begin{figure}[H]
% \centering
% \begin{subfigure}[t]{0.2\textwidth}
% \centering
% \begin{tikzpicture}
%     \node[main node] (0) {$a$};
%     \node[main node] (1) [below = 1.16cm of 0] {$b$};
%     \node[main node] (2) [below left = 0.58cm and 1cm of 1]  {$c$};
%     \node[main node] (3) [below right = 0.58cm and 1cm of 1] {$d$};

%     \path[draw,thick]
%     (0) edge node {} (1)
%     (1) edge node {} (2)
%     (1) edge node {} (3);
% \end{tikzpicture}
% \end{subfigure}
% \begin{subfigure}[t]{0.5\textwidth}
% \centering
% \begin{tikzpicture}
%     \node[main node] (0) {$a$};
%     \node[main node] (1) [below = 1.16cm of 0] {$b$};
%     \node[main node] (2) [below left = 0.58cm and 1cm of 1]  {$c$};
%     \node[main node] (3) [below right = 0.58cm and 1cm of 1] {$d$};

%     \path[draw,thick]
%     (0) edge node {} (1)
%     (1) edge node {} (2)
%     (1) edge node {} (3)
%     (2) edge node {} (3);
% \end{tikzpicture}
% \end{subfigure}
% \begin{subfigure}[t]{0.2\textwidth}
% \centering
% \begin{tikzpicture}
%     \node[main node] (0) {$a$};
%     \node[main node] (1) [below = 2cm of 0] {$b$};
%     \node[main node] (2) [right = 2cm of 1]  {$c$};
%     \node[main node] (3) [above = 2cm of 2] {$d$};

%     \path[draw,thick]
%     (0) edge node {} (1)
%     (1) edge node {} (2)
%     (2) edge node {} (3)
%     (3) edge node {} (0);
% \end{tikzpicture}
% \end{subfigure}
% \bigskip
% \vspace{2ex}
% \begin{subfigure}[t]{0.2\textwidth}
% \centering
% \begin{tikzpicture}
%     \node[main node] (0) {$a$};
%     \node[main node] (1) [below = 1.16cm of 0] {$b$};
%     \node[main node] (2) [below left = 0.58cm and 1cm of 1]  {$c$};
%     \node[main node] (3) [below right = 0.58cm and 1cm of 1] {$d$};

%     \path[draw,thick]
%     (0) edge node {} (1)
%     (1) edge node {} (2)
%     (1) edge node {} (3)
%     (0) edge node {} (2)
%     (0) edge node {} (3)
%     (2) edge node {} (3);
% \end{tikzpicture}
% \end{subfigure}
% \begin{subfigure}[t]{0.5\textwidth}
% \centering
% \begin{tikzpicture}
%     \node[main node] (0) {$a$};
%     \node[main node] (1) [right = 1cm of 0] {$b$};
%     \node[main node] (2) [right = 1cm of 1]  {$c$};
%     \node[main node] (3) [right = 1cm of 2] {$d$};

%     \path[draw,thick]
%     (0) edge node {} (1)
%     (1) edge node {} (2)
%     (2) edge node {} (3);
% \end{tikzpicture}
% \end{subfigure}
% \begin{subfigure}[t]{0.2\textwidth}
% \centering
% \begin{tikzpicture}
%     \node[main node] (0) {$a$};
%     \node[main node] (1) [below = 2cm of 0] {$b$};
%     \node[main node] (2) [right = 2cm of 1]  {$c$};
%     \node[main node] (3) [above = 2cm of 2] {$d$};

%     \path[draw,thick]
%     (0) edge node {} (1)
%     (1) edge node {} (2)
%     (2) edge node {} (3)
%     (3) edge node {} (0)
%     (0) edge node {} (2);
% \end{tikzpicture}
% \end{subfigure}
% % \includegraphics[width=0.3\linewidth]{star.jpg}
% \caption{Connected graphs of size 4}\label{fig:star}
% \end{figure}
% \begin{lemma}
% There exists estimators to recover the edge weights for all possible connected sub-graphs on 4 nodes.
% \end{lemma}
% \begin{proof}
% We will use the star and line primitives to recover the weights of the given subgraphs as follows:
% \begin{itemize}
%     \item Graph (1): We use the star structure with node $b$ as the star vertex to learn the weights of all the edges.
%     \item Graph (2): We use the star structure with node $b$ as the star vertex to learn the weights of all edges adjacent to $b$. To recover the weights of edge $(c,d)$, we use the line structure on $a-b-c-d$ rooted at $c$.
%     \item Graph (3): We use the line structure on $a-b-c-d$ rooted at $b$ and the line structure $c-d-a-b$ rooted at $c$ to recover the remaining edge.
%     \item Graph (4): We use the star structure with each of the nodes as the star vertices to learn the weights of all edges.
%     \item Graph (5): We use the line structure on $a-b-c-d$ rooted at $b$ to recover all the edges.
%     \item Graph (6): We use the star structure with nodes $a$ and $c$ as star vertices to learn the weights of all edges.
% \end{itemize}
% Sign consistency can be ensured by selecting a sign of one edge and fixing the others using \ref{lem:sign}. \textbf{}Note that the other edges in the graph do not affect our estimates since we only use maximum 2 length paths.
% \end{proof}
\end{comment}


\begin{algorithm}
	\caption{Learn the weights of undirected edges of any mixture of connected graphs.}\label{algo:generalGraph}
	\hspace*{\algorithmicindent} \textbf{Input} Vertex set $V$\\
	\hspace*{\algorithmicindent} \textbf{Output} Edge weights for the two epidemics graphs
	\begin{algorithmic}[1]
		% \State $W = \emptyset$
		\State \textcolor{gray}{//Identify the edges of the underlying graph.}
		\State $E \leftarrow \textsc{LearnEdges}(V)$
		\State \textcolor{gray}{// Learn the edge weights for 2 nodes.}
		% \State Select $S \subseteq V$ such that $|S| = 4$ and the subgraph on $S$ is connected
		\State $S, W \leftarrow \textsc{Learn2Nodes}(V, E)$
		\While {$S \neq V$}
		\State Select $u \in S, v \in V \backslash S$ such that $(u,v) \in E$
		\State \textcolor{gray}{// If $u$ has degree 3 or greater, we use the star primitive.}
		\If {deg(v) $\geq$ 3}
		\State $W \leftarrow W \cup \textsc{LearnStar}(v, E, W)$
		
		\EndIf
		\State \textcolor{gray}{// If $u$ has degree 2, we use the line primitive.}
		\If{deg(v) = 2}
		\State Set $w \in S$ such that $(u, w) \in E$
		\State Set $t \in V$ such that $(v, t) \in E$ and $t \ne u$
		\If {$t \not \in S$}
		% \State \textcolor{gray}{//Case 1: Line primitive from Section \ref{sec:line}}
		\State $W \leftarrow W \cup \textsc{LearnLine}(t, v, u, w, S, W)$
		\EndIf
		\EndIf
		\State \textcolor{gray}{// If $u$ has degree 1, we have already learned its edge.}
		\State $S \leftarrow S \cup \{v\}$
		\EndWhile
		% \EndIf
		\State Return $W$
	\end{algorithmic}
\end{algorithm}





\subsubsection{Correctness of Algorithm~\ref{algo:generalGraph}}

To prove the correctness of the main algorithm, we show the following invariant:

\begin{lemma}\label{lem:invariant}
	At any point in the algorithm, the entire neighborhood of any node of $S$ has been learned and recorded in $W$:
	$$\forall u \in S, ~\forall v \in V,  ~ (u,v) \in E \implies (u,v) \in W.$$
\end{lemma}

\vspace{-0.4cm}
\begin{proof}
	We prove the above by induction on the iteration of the while loop. Note that  by Lemma \ref{lem:learn2nodes}, after calling $\textsc{Learn2Nodes}$, $W$ contains all edges adjacent to the two vertices in $S$. Hence the base case is true. Let us assume that after $k$ iterations of the loop, the induction hypothesis holds. %We will show that at $S\cup \{v\}$ satisfies the induction hypothesis. 
		If: \\
		$\bullet$ $deg(v) \geq 3$: By Corollary \ref{corollary:LearnStar}, we recover all edges adjacent to the star vertex $v$ by using \textsc{LearnStar}. Sign consistency is ensured using edge $(u,v)\in W$ since $u \in S$. \\
		$\bullet$ $deg(v) = 2$: There exists $w \in S$ such that $(u,w) \in E$ since $|S| \ge 2$ and is connected. Since $deg(v) = 2$, there exists $t \ne u$ such that $(t, v) \in E$. Now if $t \in S$ then $(t,v) \in W$ and we are done. If $t \not \in S$ then $v$ is a line vertex for $t-v-u-w$. Corollary \ref{corollary:LearnLine} guarantees recovery of all edges on the line by using \textsc{LearnLine}. Sign consistency is ensured through edge $(v,u)$.\\
		$\bullet$ $deg(v) = 1$: Since $u \in S$, we have $(u,v) \in W$, so we are done.

	Thus by induction, after every iteration of the for loop, the invariant is maintained.
\end{proof}

\begin{theorem}\label{thm:main}
Suppose Condition \ref{ass:necessary} and \ref{ass:main} are true, Algorithm \ref{algo:generalGraph} learns the edge weights of the two mixtures in the setting of infinite samples.
\end{theorem}

\vspace{-0.4cm}
\begin{proof}
Since at every iteration, the size of $S$ increases by 1, after at most $|V|$ iterations, we have $S = V$. Using the above lemma we have that $W$ contains all the edges of the graph.
\end{proof}


\subsubsection{Finite Sample Complexity}
\input{files/sample-v3}

==> files/lower-v3.tex <==
If we assume correlation decay ($i.e.$ $\forall i \in V, ~\sum_{k \in V} p_{ki} < 1 - \gamma$ and $\forall i \in V, ~\sum_{k \in V} q_{ki} < 1 - \gamma$ ), we prove the following lower bound (see Supplemental materials \ref{app:lowerBound}):

\begin{theorem}
	We need at least $\Omega\left( \gamma \frac{N \log \left(\frac{1}{\epsilon} \right)}{\log(N)} \right)$ samples to learn a mixture of graphs that have correlation decay from epidemic cascades within precision $\epsilon$.
\end{theorem}

==> supplemental_arxiv.tex <==
\renewcommand*{\thedefinition}{\Alph{definition}}
\renewcommand*{\thetheorem}{\Alph{theorem}}
\renewcommand*{\thelemma}{\Alph{lemma}}
\renewcommand*{\thecorollary}{\Alph{corollary}}
\renewcommand*{\theclaim}{\Alph{claim}}
\renewcommand*{\thealgorithm}{\Alph{algorithm}}

\section{Preliminaries}
\subsection{Counterexamples}\label{app:counterExamples}
Let $G=(V, E_1 \cup E_2)$ be the union of the graphs from both mixtures.  In this subsection, we prove it is impossible to learn the weights of $E_1$ and $E_2$ if $G$ has less than three edges:

\paragraph{One edge:} For a graph on two nodes, we have already seen that the cascade distribution are identical if $p_{12} = \beta = 1 - q_{12}$, for any value of $\beta$, which proves the problem is not solvable.

\paragraph{Two edges:} When we have two nodes and two edges, we can without loss of generality assume that node 1 is connected to node 2 and node 3. Then, if:
\begin{itemize}
	\item $p_{12} = \beta$
	\item $q_{12} = 1 - \beta$
	\item $p_{13} = \frac{ \frac{1}{2} - \frac{\beta}{2} + \frac{1}{4}}{\frac{1}{2} - \beta}$
	\item $q_{13} = \frac{\frac{1}{4} - \frac{\beta}{2}}{\frac{1}{2} - \beta}$
\end{itemize}
The cascade distribution is identical for any value of $\beta < \frac{1}{2}$. By simple calculations, we can show the following,
\begin{itemize}
	\item Fraction of cascades with only node 1 infected: $\frac{1}{12}$.
	\item Fraction of cascades with only node 2 infected: $\frac{1}{6}$.
	\item Fraction of cascades with only node 3 infected: $\frac{1}{6}$.
	\item Fraction of cascades where 3 infected 1, but 1 did not infect 2: $\frac{1}{12}$.
	\item Fraction of cascades where 3 infected 1, 1 infected 2: $\frac{1}{12}$.
	\item Fraction of cascades where 1 infected 3, but 1 did not infect 2: $\frac{1}{12}$.
	\item Fraction of cascades where 1 infected 2, but 1 did not infect 3: $\frac{1}{12}$.
	\item Fraction of cascades where 1 infected 3 and 2: $\frac{1}{12}$.
	\item Fraction of cascades where 2 infected 1, but 1 did not infect 3: $\frac{1}{12}$.
	\item Fraction of cascades where 2 infected 1, then 1 infected 3: $\frac{1}{12}$.
\end{itemize}
Since the distribution of cascades is the same for any value of $\beta < \frac{1}{2}$, the problem is not solvable.

\subsection{Mixtures which are not well-separated} \label{app:nonDistinct}
In this section, we show how to detect and deduce the weights of edges which have the same weight across both component of the mixture. We assume  both $G_1$ and $G_2$ follow Conditions \ref{ass:necessary} and  \ref{ass:main} if we remove all non-distinct edges, and in particular  remain connected.

Suppose there exists an edge $(i,j)$ in the graph, such that $p_{ij} = q_{ij} > 0$. Then in particular, there exists another edge connecting $i$ to the rest of the graph $G_1$ through node $k$, such that $p_{ik} \neq q_{ik}$. Then:

\begin{lemma}
	Suppose $G_1$ and $G_2$ follow assumption \ref{ass:main} after removing all non-distinct edges. We can detect and learn the weights of non-distinct edges the following way:
	
	If  $X_{ij} > 0$, and $\forall k \in V, ~X_{ik} >0 \implies Y_{ik, ij} - X_{ik}X_{ij} = 0$, then $p_{ij} = q_{ij} = X_{ij}$.
\end{lemma}
\begin{proof}
Since $G_1$ is connected on three nodes or more even when removing edge $(i,j)$, we know there exists a node $l$ such either $l$ is connected to either $i$ or $k$. Therefore, either $Y_{ik, il} - X_{ik}X_{il} > 0$ or $Y_{ki, kl} - X_{ki}X_{kl} > 0 $. In both these cases, we deduce $p_{ik} \neq q_{ik}$. This in turns allow us to detect that $p_{ij} = q_{ij}$. Once this edge is detected, it is very easy to deduce its weight, since $p_{ij} = X_{ij} = q_{ij}$ by definition.
\end{proof}


\section{Proofs for unbiased mixtures}
\subsection{Estimators - proofs}
\begin{lemma}\label{app:line}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, the weights of the edges for a line structure are then given by: 
	\begin{align*}
	p_{ua} &= X_{ua} + s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub})R^| }{Y^|_{ub, bc} - X_{ua}X_{bc}}},~q_{ua} = X_{ua} - s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub})R^| }{Y^|_{ub, bc} - X_{ua}X_{bc}}}, \\
	p_{bc} &= X_{uc} + s_{bc} \sqrt{\frac{(Y^|_{ub, bc} - X_{ua}X_{bc})R^| }{Y^|_{ua,ub} - X_{uc}X_{ua}}},~q_{bc} = X_{uc} - s_{bc} \sqrt{\frac{(Y^|_{ub, bc} - X_{ua}X_{bc})R^| }{Y^|_{ua,ub} - X_{uc}X_{ua}}}\\
	p_{ub} &= X_{ub} + s_{ub} \sqrt{\frac{(Y^|_{uc,ua} - X_{uc}X_{ua})(Y^|_{ub, bc} - X_{ua}X_{bc})}{R^|}}, \\
	q_{ua} &= X_{ua} - s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{uc}X_{ua})(Y^|_{ub, bc} - X_{ua}X_{bc})}{R^|}}, \\
	\end{align*}
	where $R^| = X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}$, and for $s_{ua} \in \{-1,1\}$.
\end{lemma}
\begin{proof} 
	In this case, there is no edge between $u$ and $c$, which implies that $p_{uc} = q_{uc} = 0$.  Hence, we cannot use a variation of the equation above for finding the edges of a star structure without dividing by zero. Therefore, we need to use $Z^|_{ua, ub, bc}$. 
	Let $R^| = X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}$. We notice a remarkable simplification:
	\begin{align*}
	R^| &= X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}} \\
	&= \frac{p_{ua} + q_{ua}}{2}\cdot\frac{p_{bc} + q_{bc}}{2} + \frac{\frac{p_{ua}p_{ub}p_{bc} + q_{ua}q_{ub}q_{bc}}{2} - \frac{p_{ua} + q_{ua}}{2} \cdot \frac{p_{ua}p_{bc} + q_{ua}q_{bc}}{2} - \frac{p_{bc} + q_{bc}}{2}\cdot\frac{p_{ua}p_{ua} + q_{ua}q_{ua}}{2}}{\frac{p_{ub} + q_{ub}}{2}} \\
	&= \frac{1}{4} (p_{ua}p_{bc} + p_{ua}q_{bc} + q_{ua}p_{bc} + q_{ua}q_{bc}) + \frac{2}{p_{ub} + q_{ub}}\left[\frac{p_{ua}p_{ub}p_{bc} + q_{ua}q_{ub}q_{bc}}{2}  \right.\\
	&\quad \left.- \frac{1}{4}(p_{ua}p_{ub}p_{bc} + q_{ua}p_{ub}p_{bc} + p_{ua}q_{ub}q_{bc} + q_{ua}q_{ub}q_{bc}) \right.\\
	&\quad \left. -\frac{1}{4}(p_{ua}p_{ub}p_{bc} + p_{ua}p_{ub}q_{bc} +  q_{ua}q_{ub}p_{bc} + q_{ua}q_{ub}q_{bc})\right] \\
	&= \frac{1}{4} (p_{ua}p_{bc} + p_{ua}q_{bc} + q_{ua}p_{bc} + q_{ua}q_{bc}) - \frac{1}{2(p_{ub} + q_{ub})}\left[q_{ua}p_{ub}p_{bc} + p_{ua}q_{ub}q_{bc} + p_{ua}p_{ub}q_{bc} +  q_{ua}q_{ub}q_{bc} \right] \\
	&= \frac{1}{4} (p_{ua}p_{bc} + q_{ua}p_{bc} + q_{ua}q_{bc}+ p_{ua}q_{bc} )  - \frac{1}{2(p_{ub} + q_{ub})}\left[(p_{ub} + q_{ub})( q_{ua}p_{bc} + p_{ua}q_{bc}) \right] \\
	&= \frac{1}{4}(p_{ua}p_{bc} + q_{ua}q_{bc} - p_{ua}q_{bc} - q_{ua}p_{bc}) \\
	&= \frac{1}{4}(p_{ua} - q_{ua})(p_{bc} - q_{bc})
	\end{align*}
	
	We can then use the same proof techniques as in Lemma \ref{lem:star}, and finally obtain:
	\begin{align*}
	|p_{ua} - q_{ua}| &= \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ua})\left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}\right) }{Y^|_{ub, bc} - X_{ua}X_{bc}}}.
	% , \\
	% |p_{ub} - q_{ub}| &= \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub})(Y^|_{ub, bc} - X_{ua}X_{bc})}{\left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}\right)}}, \\
	% |p_{bc} - q_{bc}| &= \sqrt{\frac{(Y^|_{ub, bc} - X_{ua}X_{bc})\left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}\right) }{Y^|_{ua,ub} - X_{ua}X_{ua}}}.
	\end{align*}
	This gives us the required result.
\end{proof}

\subsection{Main algorithm - proofs} \label{app:algo}
Here we will present in detail the sub-routines required by our algorithm and the essential lemmas needed for our main proof.
\paragraph{LearnEdges} This procedure detects the edges in the underlying graph using the estimate $X_{uv}$.
\begin{algorithm}[H] 
	\caption{$\textsc{LearnEdges}$}\label{app:learnEdges}
	\hspace*{\algorithmicindent} \textbf{Input} Vertex set $V$\\
	\hspace*{\algorithmicindent} \textbf{Output} Edges of the graph
	\begin{algorithmic}[1]
		\State Set $E \leftarrow \emptyset$
		\For {$u < v \in V$}
		\State Compute $\hat{X}_{uv}$
		\If {$\hat{X}_{uv} \ge \epsilon$}
		\State $E \leftarrow E \cup \{(u,v)\}$
		\EndIf
		\EndFor
		\State Return $E$
	\end{algorithmic}
\end{algorithm}
\begin{claim}\label{cl:Xab}
	$\textsc{LearnEdges}(V)$ outputs $E$ such that $E = E_1 \cup E_2$.
\end{claim}
\begin{proof}
	For each pair of nodes $u,v \in V$, if $(u,v) \in E_1 \cup E_2$ then $X_{uv} \ne 0$ since $X_{uv} = 0$ if and only if $p_{uv} = q_{uv} = 0$, which is equivalent to the edge $(u, v)$ not belonging in the mixture.
\end{proof}
\paragraph{LearnStar} This procedure returns the weights of the outgoing edges of a star vertex using the star primitive discussed before.
\begin{algorithm}[H] 
	\caption{$\textsc{LearnStar}$}\label{app:learnStar}
	\hspace*{\algorithmicindent} \textbf{Input} Star vertex $u \in V$, edge set $E$, weights $W$\\
	\hspace*{\algorithmicindent} \textbf{Output} Weights of edges adjacent to $u$
	\begin{algorithmic}[1]
		\State Use star primitive with star vertex $u$ and learn all adjacent edges weights $W^*$.
		\If {$W = \emptyset$}
		\State Fix sign of any edge and ensure sign consistency.
		\Else
		\State Set $v \in V$ such that $(u,v) \in W$.
		% \State Set $N = \{w \in V | (u,w) \in E, (u,w) \not \in W\}$
		\State Use $s_{uv}$ to remove sign ambiguity 
		\EndIf
		\State Return $W^*$.
	\end{algorithmic}
\end{algorithm}
% The $\textsc{LearnStar}(u,a, S, W)$ runs as follows:
% \begin{enumerate}
%     \item Using $a$ as the star node in the star structure, we use estimates to recover the edge weights of all edges adjacent to $a$ using $u$ as a fixed node.
%     \item Fix sign consistencies using $s_{ua}$.
% \end{enumerate}
\begin{lemma}\label{lem:learnstar}
	If $deg(u) \ge 3$, $\textsc{LearnStar}(u, S, W)$ recovers $p_{ua}, q_{ua}$ for all $a$ such that $(u,a) \in E$. 
\end{lemma}
\begin{proof}
	The proof follows from using Lemma \ref{lem:star} on star vertex $u$ (degree of $u \ge 3$) and using Lemma \ref{lem:sign} to resolve sign ambiguity through fixing an edge or $s_{uv}$ ($(u,v) \in W$ hence know sign). 
\end{proof}

\paragraph{LearnLine} This procedure returns the weights of the edges of a line $a-b-c-d$ rooted at vertex $b$ of degree 2 using the line primitive discussed before.
\begin{algorithm}[H] 
	\caption{$\textsc{LearnLine}$}\label{app:learnLine}
	\hspace*{\algorithmicindent} \textbf{Input} Line $a-b-c-d$ with $deg(b) = 2$, edge set $E$, weights $W$\\
	\hspace*{\algorithmicindent} \textbf{Output} Weights of edges $(a,b), (b,c), (c,d)$
	\begin{algorithmic}[1]
		\State Use line primitive on $a-b-c-d$ rooted at $b$ and learn all edges weights $W^|$.
		\If {$W = \emptyset$}
		\State Fix sign of any edge and ensure sign consistency.
		\Else
		\State Find edge $e \in \{(a,b), (b,c), (c,d)\}$ such that $e \in W$.
		% \State Set $N = \{w \in V | (u,w) \in E, (u,w) \not \in W\}$
		\State Use $s_{e}$ to remove sign ambiguity.
		\EndIf
		\State Return $W^|$.
	\end{algorithmic}
\end{algorithm}
% The $\textsc{LearnLine}(u,a, S, W)$ runs as follows:
% \begin{enumerate}
%     \item Choose vertex $c \in S$ such that $(u,c) \in E$. Choose vertex $b\ne c, u$ such that $(a,b) \in E$. If there does not exist such $b$, return empty set.
%     \item Using line structure on $c-u-a-b$ rooted at $a$, use estimates to recover the edge weights of edge $(a,b)$.
%     \item Fix sign consistencies using $s_{ua}$.
% \end{enumerate}
\begin{lemma}\label{lem:learnline}
	If $deg(b) = 2$, $\textsc{LearnLine}(a, b, c, d, S, W)$ recovers $p_{ab}, q_{ab}, p_{bc}, q_{bc}, p{cd}, q_{cd}$. 
\end{lemma}
\begin{proof}
	The proof follows from using Lemma \ref{lem:line} on line $a-b-c-d$ rooted at vertex $b$ (degree of $b= 2$) and using Lemma \ref{lem:sign} to resolve sign ambiguity by fixing an edge or using $s_{e}$.
\end{proof}

\paragraph{Learn2Nodes} This procedure chooses a pair of connected vertices in our graph and outputs the weights of all outgoing edges of each of the two vertices. We initialize our algorithm using this procedure.
\begin{algorithm}[H] 
	\caption{$\textsc{Learn2Nodes}$}\label{app:learn2Nodes}
	\hspace*{\algorithmicindent} \textbf{Input} Vertex set $V$, Edge Set $E$\\
	\hspace*{\algorithmicindent} \textbf{Output} Set of 2 vertices $V$, Weight of all edges adjacent to the vertices $W$
	\begin{algorithmic}[1]
		\State $W = \emptyset$
		\State Set $u = \argmax_{a \in V} deg(a)$
		\State Set $v = \argmin_{a \in V, (u,a) \in E} deg(a)$
		\If {$deg(u) \ge 3$}
		\State $W \leftarrow \textsc{LearnStar}(u, E, W)$
		\If {$deg(v) = 3$}
		\State $W \leftarrow W \cup \textsc{LearnStar}(v, E, W)$
		\ElsIf {$deg(v) = 2$}
		\State Let $t \in V$ be such that $(t, v) \in E$ and $t \ne u$
		\State Let $w \in V$ be such that $(w, u) \in E$ and $w \ne v,t$
		\If {$v = t$}
		\State $W \leftarrow W \cup \textsc{LearnLine}(t, v, u, w, W)$
		\EndIf
		\EndIf
		\Else
		\State $w$ be such that $(w, u) \in E$ and $w \ne v$
		\If {$deg(v) = 2$}
		\State Let $t \in V$ be such that $(t, v) \in E$ and $t \ne u$
		\State $W \leftarrow \textsc{LearnLine}(w, u, v, t, W)$
		\Else
		\State Let $t \in V$ be such that $(t, w) \in E$ and $t \ne w$
		\State $W \leftarrow \textsc{LearnLine}(v, u, w, t, W)$
		\EndIf
		\EndIf
		\State Return $(u,v), W$
	\end{algorithmic}
\end{algorithm}
\begin{lemma} \label{lem:learn2nodes}
	Under Conditions \ref{ass:necessary} and \ref{ass:main}, $\textsc{Learn2Nodes}(V)$ outputs two connected nodes $(u,v)$ and weights of all edges adjacent to $u,v$.
\end{lemma}
\begin{proof}
	We will break the proof down into cases based on the degree of chosen vertices $u,v$ as follows,
	\begin{itemize}
		\item $deg(u) \ge 3$: By Lemma \ref{lem:learnstar}, we can recover all the edges of $u$ and fix a sign.
		\begin{itemize}
			\item $deg(v) \ge 3$: By Lemma \ref{lem:learnstar}, we can recover all the edges of $v$ and ensure sign consistency by using the edge $(u,v)$.
			\item $deg(v) = 2$: Since $deg(v) = 2$, there exists a vertex $t \ne u$ such that $(t,u) \in E$. Since $deg(u) \ge 3$, there must exist $w \ne t, u$ such that $(u,w) \in E$. Now we have line primitive $t-v-u-w$  with $deg(v) = 2$ and Lemma \ref{lem:learnline} guarantees recovery of the edge weights.
			\item $deg(v) = 1$, then we already know all the edges adjacent to $v$.
		\end{itemize}
		\item $deg(u) = 2, deg(v) = 2$: Since the max degree of the graph is 2 and it is connected then it can either be a line or a cycle. There are at least 4 nodes in the graph, thus there exist $w \ne v$ such that $(w, u) \in E$ and $t \ne u, w$ such that $(v,t) \in E$. This gives a path $w-u-v-t$ with $deg(u) = 2$ and Lemma \ref{lem:learnline} guarantees recovery of all edges.
		\item $deg(u) = 2, deg(v) = 1$: As in the previous case, the underlying graph is a line. Therefore there exist path $v-u-w-t$ and we can similarly apply Lemma \ref{lem:learnline} to guarantee recovery of all edges. 
	\end{itemize}
\end{proof}





\subsection{Finite sample complexity - proofs} \label{app:finiteSamples}
In this section, we provide explicit proof for the sample complexity of our algorithm. To do so, we bound below the number of cascades starting on each node through Bernstein inequality, and use this number to obtain concentration of all the estimators.


\begin{definition}
	Among $M$ cascades, let $M_u$ be the number of times node $u$ is the source.
\end{definition}

\begin{claim}\label{cl:Mu}
	With $M$ samples, every node is the source of the infection at least $\frac{M}{2N}$ times with probability at least $1- e^{-\frac{3M}{26N}}$.
\end{claim}
\proof  Among $M$ cascade, the expectation of $M_u$ is $\frac{M}{N}$, since the source is chosen uniformly at random among the $N$ vertices of $V$. Since $M_u$ can be seen as the sum of Bernoulli variable of parameter $\frac{1}{N}$, we can use Bernstein's inequality to bound it below:
\begin{align*}
\Pr(M_u < \frac{M}{2N}) &= \Pr\left(\frac{M}{N} - M_u > \frac{M}{2N}\right)\\
&\leq e^{ - \frac{\left(\frac{M}{2N}\right)^2}{2M\frac{1}{N}(1- \frac{1}{N}) + \frac{1}{3}\frac{M}{2N}}} \\
&\leq e^{-\frac{3M}{26N}}.
\end{align*}

\begin{claim}\label{cl:epsilon1}
	Let $u$ either be a star vertex, with neighbors $a, b$ and $c$, or be part of a line structure rooted in $u$, with neighbors $a, b$, and $c$ neighbor of $b$. Suppose $M_u \geq \frac{M}{2N}$. Then with $M = \frac{N}{\epsilon^2} \log\left(\frac{12N^2}{\delta}\right)$ samples, with probability at least $1- \frac{\delta}{6N^2}$, we can guarantee any of the following:
	\begin{enumerate}
		\item $\forall r \in {a,b,c}, ~ \left|\hat{X}_{ur} - X_{ur}\right| \le  \epsilon_1 $.
		\item $\forall r \neq s \in \{a,b,c\}, ~|\hat{Y}^*_{ur,us} - \hat{Y}^*_{ur,us}| \le  \epsilon_1$.
		\item $|\hat{Y}^|_{ua,ub} - \hat{Y}^|_{ua,ub}| \le  \epsilon_1$ and $|\hat{Y}^|_{ua,ab} - \hat{Y}^|_{ua,ab}| \le  \epsilon_1$.
		\item $|\hat{Z}^|_{ua,ub,bc} - Z^|_{ua,ub,bc}| \le \epsilon_1$.
	\end{enumerate}
\end{claim}
\proof By Hoeffding's inequality:
\begin{align*}
\Pr( |\hat{X}_{ur} - X_{ur}| >  \epsilon_1) &= \Pr\left( \left|\sum_{m =1}^{M_u} \mathbb{1}_{\{u \rightarrow r~|~ u \in I_0\}} - M_u\cdot X_{ur} \right| >  M_{u}\cdot \epsilon_1 \right) \\
&\leq \Pr\left( \left|\sum_{m =1}^{\frac{M}{2N}} \mathbb{1}_{\{u \rightarrow r~|~ u \in I_0\}} - \frac{M}{2N}\cdot X_{ur} \right| >  \frac{M}{2N} \cdot \epsilon_1 \right) \\
&\leq \displaystyle 2e^{-2\frac{M}{2N}\epsilon_1^2}.
\end{align*}
Therefore, the quantity above is smaller than $\frac{\delta}{6N^2}$ for $M \geq \frac{N}{\epsilon_1^2} \log\left(\frac{12N^2}{\delta}\right)$. The proof is almost identical for the other quantities involved.

\begin{claim}\label{cl:epsilon2}
	If we can estimate $X_{ua}, Y^*_{ua,ub}, Y^|_{ua,ab}$ and $Z^|_{ua,ub,bc}$ within $\epsilon_1$, we can estimate $p_{ua}$ within precision $\epsilon = \frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1$.
\end{claim}
\proof 
If $u$ is of degree three or more, we use a star primitive to estimate it. Let $a, b$ and $c$ be three of its neigbors:
\begin{align*}
\hat{p}_{ua} &=  \hat{X}_{ua} + s_{ua} \sqrt{\frac{(\hat{Y}_{ua,ub} - \hat{X}_{ua}\hat{X}_{ub})(\hat{Y}_{ua,uc} - \hat{X}_{ua}\hat{X}_{uc})}{\hat{Y}_{ub,uc} - \hat{X}_{ub}\hat{X}_{uc}}} \\
&\leq X_{ua} + \epsilon_1 \\
&\quad+ s_{ua} \left(\frac{(Y_{ua,ub} - X_{ua}X_{ub} + s_{ua}\left(1 + X_{ua} + X_{ub}\right)\epsilon_1)(Y_{ua,uc} - X_{ua}X_{uc} + s_{ua}\left[1 + X_{ua} + X_{uc}\right)\epsilon_1) }{Y_{ub, bc} - X_{ub}X_{uc} - s_{ua}\left(1 + X_{ub} + X_{uc}\right)\epsilon_1)}\right]^\frac{1}{2} \\
&\leq X_{ua} + \epsilon_1 +  s_{ua} \sqrt{\frac{(Y_{ua,ub} - X_{ua}X_{ub})(Y_{ua,uc} - X_{ua}X_{uc})}{Y_{ub,uc} - X_{ub}X_{uc}}}\left(\frac{(1 + s_{ua}\frac{3\epsilon_1}{\frac{\Delta^2}{4}})^2}{1 - s_{ua}\frac{3\epsilon_1}{\frac{\Delta^2}{4}}} \right)^\frac{1}{2} \\
&\leq p_{ua} + \epsilon_1 + p_{ua} \left( \frac{12}{\Delta^2} + \frac{6}{\Delta^2}\right)\cdot \epsilon_1 + o(\epsilon_1) \\
&\leq p_{ua} + \frac{19}{\Delta^2}\cdot \epsilon_1 + o(\epsilon_1).
\end{align*}
Where we have used $Y_{ur,us} - X_{ur}X_{us} \geq \frac{\Delta^2}{4}$, $s_{ua}^2 = 1$, $p_{ua} \leq 1$, $1 \leq \frac{1}{\Delta^2}$. We then conclude by symmetry.

If $u$ is of degree two, we use a line primitive to estimate it:
\begin{align*}
\hat{p}_{ua} &= \hat{X}_{ua} + s_{ua} \sqrt{\frac{(\hat{Y}^|_{ua,ub} - \hat{X}_{ua}\hat{X}_{ub})\left(\hat{X}_{ua}\hat{X}_{bc} + \frac{\hat{Z}^|_{ua, ub, bc} - \hat{X}_{ua}\hat{Y}^|_{ub, bc} - \hat{X}_{bc}\hat{Y}^|_{ua,ub}}{\hat{X}_{ub}}\right) }{\hat{Y}^|_{ub, bc} - \hat{X}_{ua}\hat{X}_{bc}}}\\
&\leq X_{ua}  + \epsilon_1 + s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub} + 3s_{ua}\epsilon_1)\left(X_{ua}X_{bc} + 2\epsilon_1 + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub} + 5s_{ua}\epsilon_1 }{X_{ub} - s_{ua}\epsilon_1 } \right) }{Y^|_{ub, bc} - X_{ua}X_{bc} - 3s_{ua}\epsilon_1}}.
\end{align*}
As shown in the proof of Lemma \ref{lem:line}, we have:
\begin{align*}
Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}   &= \frac{1}{2}(p_{ub} + q_{ub})(q_{ua}p_{bc} + p_{ua}q_{bc}) \\
&\geq \frac{p^3_{min}}{2} \\
\left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}} \right) &= \frac{1}{4}(p_{ua} - q_{ua})(p_{bc} - q_{bc}) \\
&\geq \frac{\Delta^2}{4}.
\end{align*}
Therefore:
\begin{align*}
\frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub} + 5s_{ua}\epsilon_1 }{X_{ub} - s_{ua}\epsilon_1 } &\leq      \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub} }{X_{ub}}  \left[ \frac{1 + s_{ua}\frac{5\epsilon_1}{\frac{p^3_{min}}{2}}}{1 - s_{ua}\frac{\epsilon_1}{\frac{p_{min}}{2}}} \right] \\
&\leq  \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}} + s_{ua}\left( \frac{12}{p^3_{min}}\right) \epsilon_1 + o(\epsilon_1).
\end{align*}
We also have:
\begin{align*}
X_{ua}X_{bc} + 2\epsilon_1 + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub} + 5s_{ua}\epsilon_1 }{X_{ub} - s_{ua}\epsilon_1 } &\leq \left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}} \right) 
\\&\quad \cdot \left(1 + s_{ua}\frac{\frac{14}{p_{min}^3}}{\frac{\Delta^2}{4}}\epsilon_1 \right) + o(\epsilon_1).
\end{align*}
Combining all the above inequalitites:
\begin{align*}
\hat{p}_{ua} &\leq X_{ua} + \epsilon_1 + s_{ua} \sqrt{\frac{(Y^|_{ua,ub} - X_{ua}X_{ub})\left(X_{ua}X_{bc} + \frac{Z^|_{ua, ub, bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}}{X_{ub}}\right) }{Y^|_{ub, bc} - X_{ua}X_{bc}}} \\
&\quad\cdot\left[ \frac{\left(1 + \frac{3\epsilon_1}{\frac{\Delta^2}{4}}\right)\left(1 + s_{ua}\frac{\frac{14}{p_{min}^3}}{\frac{\Delta^2}{4}}\epsilon_1 \right)}{1 - s_{ua}\frac{3\epsilon_1}{\frac{\Delta^2}{4}}} \right]^\frac{1}{2} \\
&\leq p_{ua} + \epsilon_1 + p_{ua}s_{ua}^2\left( \frac{6}{\Delta^2} + \frac{28}{p_{min}^3\Delta^2} + \frac{6}{\Delta^2} \right)\cdot \epsilon_1 + o(\epsilon_1) \\
&\leq p_{ua} + \frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1 + o(\epsilon_1).
\end{align*}
We can conclude by symmetry. 

Since $\frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1 \geq \frac{19}{\Delta^2}\cdot \epsilon_1$, we conclude that we can know $p_{ua}$ within precision $\epsilon = \frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1$ regardless of the degree of $u$.

\begin{theorem}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main},, with probability $1- \delta$, with $M = N\cdot\frac{ 41^2}{p_{min}^{6}\Delta^4\cdot \epsilon^2} \log\left( \frac{12N^2}{\delta}\right) = \OO\left( \frac{N}{\epsilon^2}\log\left( \frac{N}{\delta}\right) \right)$ samples, we can learn all the edges of the mixture of the graphs within precision $\epsilon$.
\end{theorem}
\proof 
We pick $\epsilon = \frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1$. We use Claim \ref{cl:Mu} to bound the quantity $\Pr( M_u < \frac{M}{2N})$, and Claim \ref{cl:epsilon1} and \ref{cl:epsilon2} to bound $\Pr(|\hat{p}_{ua} - p_{ua}| > \frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1 | M_u \geq \frac{M}{2N})$.  For $(u,a)$ edge of the graph:
\begin{align*}
\Pr(|\hat{p}_{ua} - p_{ua}| > \epsilon) &\leq \Pr(|\hat{p}_{ua} - p_{ua}| > \epsilon | M_u < \frac{M}{2n})\cdot \Pr( M_u < \frac{M}{2N}) \\
&\quad+ \Pr(|\hat{p}_{ua} - p_{ua}| > \epsilon | M_u \geq \frac{M}{2n})\cdot \Pr( M_u \geq \frac{M}{2N}) \\
&\leq 1\cdot \displaystyle 2e^{-2\frac{M}{2N}}  + \Pr(|\hat{p}_{ua} - p_{ua}| > \epsilon | M_u \geq \frac{M}{2N})\cdot 1 \\
&\leq \frac{\delta}{12N^2} + \Pr(|\hat{p}_{ua} - p_{ua}| > \frac{41}{p_{min}^3\Delta^2}\cdot \epsilon_1 | M_u \geq \frac{M}{2N}) \\
&\leq \frac{\delta}{12N^2} + \frac{\delta}{12N^2} \\
&\leq \frac{\delta}{6N^2}.
\end{align*}
We conclude by union bound on the six estimators involved for all the pairs of nodes in the graph, for a total of at most $6N^2$ estimators.



\subsection{Complete graph on three nodes} \label{app:triangle}
In this section, we prove it is possible to recover the weights of a mixture on three nodes, as long as there are at least three edges in $E_1 \cup E_2$. Since no node is of degree 3, no node is a star vertex, and since there are less than four nodes, no node is a line vertex, and we can not use the techniques developped above for connected graphs on four vertices or more. However, we can still use very similar proofs techniques. Suppose the vertices of $V$ are $1$, 2 and 3.
\begin{definition}
	 We reuse the quantities defined for star vertices:
	\begin{itemize}
		\item For $i$, $j$ distinct in $\{1,2,3 \}, ~\hat{X}_{ij} =  \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{i \rightarrow j, i \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{i \in I_0^m}} \to_{M \to \infty} X_{ij} = \frac{p_{ij} + q_{ij}}{2}.$
		\item For $i$, $j$, $k$ distinct in $\{1,2,3 \}, ~Y_{ij,ik} = \frac{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{i \rightarrow j, i \rightarrow k, i \in I_0^m}}{\frac{1}{M}\sum_{m = 1}^M \mathbb{1}_{u \in I_0^m}} \to_{M \to \infty} Y_{ij, ik}= \frac{p_{ij}p_{ik} + q_{ij}q_{ik}}{2}.$
	\end{itemize}
\end{definition}
Even though neither 1, 2 or 3 is a star vertex, we can write the same kind of system of equations as a star vertex would satisfy. In particular:

$$\frac{|p_{ij} - q_{ij}|}{2} = \sqrt{\frac{(Y_{ij,ik} - X_{ij}{ik})(Y_{ji, jk} - X_{ji}X_{jk})}{Y_{ki,kj} - X_{ki}X_{kj}}}. $$

Resolving the sign ambiguity as previoulsy (Lemma \ref{lem:sign}), this finally yields:

\begin{align*}
p_{ij} &= X_{ij} + s_{ij}\sqrt{\frac{(Y_{ij,ik} - X_{ij}{ik})(Y_{ji, jk} - X_{ji}X_{jk})}{Y_{ki,kj} - X_{ki}X_{kj}}}, \\
q_{ij} &= X_{ij} + s_{ij}\sqrt{\frac{(Y_{ij,ik} - X_{ij}{ik})(Y_{ji, jk} - X_{ji}X_{jk})}{Y_{ki,kj} - X_{ki}X_{kj}}}.
\end{align*}




\section{Lower Bound} \label{app:lowerBound}
In this section, we prove a lower bound for learning the weights of the mixture. The proof follows the general idea of \cite{Netrapalli2012}. In particular, we recall their definition of correlation decay:

\begin{definition}
	Let $G = (V,E)$ be a weighted graph with weight $r_{ij}$ for edge $(i,j)$. We say $G$ has \textbf{correlation decay} if there exists $\gamma$ such that:
	$$\forall i \in V, \sum_{k \in V} r_{ki} < 1 - \gamma . $$
\end{definition}

We define a quantity which will be useful for our analysis:
\begin{definition}
	For each edge $(i,j)$ in the graph, for each cascade $m$, we define:
$$Z_{i,j}^m = \text{Time at which $i$ infect $j$ during cascade $m$.} $$
$$Z = \{ Z_{i,j}^m \}_{i,j \in V}^{1 \leq m \leq M}. $$
Note that this time can be infinite if $i$ did not infect $j$. We also define:
$$ So^m = \text{Source of cascade $m$.}$$
$$ So = \{ So^m \}^{1 \leq m \leq M}. $$
\end{definition}

We notice that $S^m$ and $\{ Z_{ij}^m\}_{i,j \in V} $ contain all the information we get from cascade $m$. Let $\hat{G}$ be the reconstructed graph we build from all the $M$ epidemic cascades, and let $\mathcal{G}$ be the set of all possible mixture of weighted graph. Since we want to recover each edge within precision $\epsilon$, if $\epsilon < p_{min}$, we have:

$$ |\mathcal{G}| = \left(1 + \frac{1-p_{min}}{\epsilon} \right)^{\frac{N(N-1)}{2}} \geq \left(\frac{1-p_{min}}{\epsilon}\right)^{\frac{N(N-1)}{2}}$$

Suppose $G$ is drawn uniformly from $\mathcal{G}$. Let write $H(A)$ to be the entropy of the random variable $A$. Let $\delta$ be the probability that our algorithm fails. We have:

\begin{align*}
\log(|\mathcal{G}|) &= H(G)  \\
&=I(G;\hat{G}) + H(G|\hat{G}) \\
\text{(data processing inequality)} \quad &\leq I(G;So,Z) + H(G|\hat{G}) \\
\text{(independent cascades)}  \quad &\leq  M\cdot I(G;So^1, \{Z^1_{ij}\}_{i,j \in V} ) + H(G|\hat{G})\\
\text{($I(X,Y) \leq H(X)$)}  \quad &\leq  M \cdot \sum_{i,j=1, i\neq j}^N H(So^1, \{Z^1_{ij}\}_{i,j \in V} ) + H(G|\hat{G}) \\
\text{(Fano's inequality)} \quad &\leq  M\cdot \sum_{i,j=1, i\neq j}^N H(So^1, \{Z^1_{ij}\}_{i,j \in V} ) + (1 + \delta\log(|\mathcal{G}|) )  \\
(H(X,Y) \leq H(X) + H(Y) )&\leq  M\cdot \left(H(So^1) +  \sum_{i,j=1, i\neq j}^N  H(\{Z^1_{ij}\}_{i,j \in V} ) \right) + (1 + \delta\log(|\mathcal{G}|) ) 
\end{align*}

Similarly to \cite{Netrapalli2012}, we have:
\begin{claim}\label{claim:netrapalli}
	We prove the following inequalities:
	\begin{enumerate}
		\item $\Pr(Z_{ij}^1 = t+1) \leq \frac{1}{N}(1-\gamma)^t.$
		\item $H(Z^1_{ij}) \leq \frac{1}{N}\frac{6\log(N)}{\gamma(1 - \gamma)}.$
		\item $H(So^1) = \log(N).$
	\end{enumerate}

\end{claim}
\begin{proof}
	\begin{enumerate}
		\item $Z_{ij}^1 = t+1$ only if $i$ got infected at time $t$, which happens with probability at most $\frac{1}{N}(1-\gamma)^t$ thanks to correlation decay, as seen in the proof of Lemma 1 of \cite{Netrapalli2012} (in Appendix A).
		\item 	From the proof in Appendix D.1 of \cite{Netrapalli2012}, we have $H(Z^1_{ij}) \leq \frac{1}{N} \left[ \frac{1}{1-\gamma} \left( \log(N) - \left(\frac{1 - \gamma}{\gamma} \right)^2 \log(1 - \gamma) \right) - \left(1 - \frac{1}{N\gamma}\right) \log\left(1 - \frac{1}{N\gamma} \right)\right]$. Then:
		
		\begin{align*}
		H(Z^1_{ij}) &\leq \frac{1}{N} \left[ \frac{1}{1-\gamma} \left( \log(N) - \left(\frac{1 - \gamma}{\gamma} \right)^2 \log(1 - \gamma) \right) - \left(1 - \frac{1}{N\gamma}\right) \log\left(1 - \frac{1}{N\gamma} \right)\right] \\
		&\leq \frac{1}{N} \left[ \frac{1}{1-\gamma} \left( \log(N) + 2 \frac{(1 - \gamma)^2}{\gamma}   \right) + 1\cdot\frac{2}{N\gamma}\right] \\
		&\leq \frac{1}{N}\frac{6\log(N)}{\gamma(1 - \gamma)}.
		\end{align*}
		\item Finally, $So^1$ is uniformly drawn among $N$ possible values, so $H(So^1) = \log(N)$.
	\end{enumerate}

\end{proof}

Plugging Claim \ref{claim:netrapalli} into the equations above:
\begin{align*}
M &\geq \frac{(1 - \delta)\log(|\mathcal{G}|) - 1}{H(S^1) +  \sum_{i,j=1, i\neq j}^N  H(\{Z^1_{ij}\}_{i,j \in V} )} \\
&\geq \frac{(1 - \delta)\frac{N(N-1)}{2}\log(\frac{1-p_{min}}{\epsilon}) - 1}{\log(N) +  \sum_{i,j=1, i\neq j}^N  \frac{1}{N}\frac{6\log(N)}{\gamma(1 - \gamma)}} \\
&\geq \gamma(1 - \gamma)\frac{(1 - \delta)\frac{N(N-1)}{2}\log(\frac{1-p_{min}}{\epsilon}) - 1}{(N-1)7\log(N)} \\
&= \Omega\left( \gamma \frac{N \log \left(\frac{1}{\epsilon} \right)}{\log(N)} \right).
\end{align*}

We therefore have established the following lower bound:
\begin{theorem}
	We need at least $\Omega\left( \gamma \frac{N \log \left(\frac{1}{\epsilon} \right)}{\log(N)} \right)$ samples to learn a mixture of graphs that have correlation decay from epidemic cascades within precision $\epsilon$.
\end{theorem}




\section{Learning graphs with biased mixture priors with known bias $\alpha$} \label{app:unknownAlpha}

In this section we provide the primitives required for \textsc{LearnStar} and \textsc{LearnLine}, when the first mixture occurs with probability  $\alpha$ and the second mixture with probability $(1-\alpha)$. 

\textbf{Notations:} In this section, to avoid clutter in notation we use $i$, $j$ and $k$ to be all \emph{distinct} unless mentioned otherwise. Also, let $\sigma(\{a,b,c\}) =\{ (a,b,c), (b,c,a), (c, a, b)\}$ denote all the permutations of $a$, $b$, and $c$.

\begin{claim} \label{cl:genEstimators}
	If $a$ and $b$ are two distinct nodes of $V_1 \cap V_2$ such that $(a,b) \in E_1 \cap E_2$ then  under general mixture model $X_{ab} = \alpha p_{ab} + (1- \alpha) q_{ab}$. 
	
	Fuither, when the four nodes $u$, $a$, $b$ and $c$ forms a \underline{star graph} (Fig.~\ref{fig:star}) with $u$ in the center under general mixture model 
	\begin{align*}
	&1)~\forall i, j \in\{a,b,c\}, i, j\neq u, Y_{ui, uj} = \alpha  p_{ui}p_{uj} + (1- \alpha)  q_{ui}q_{uj},\\
	& 2)~ Z_{ua, ub, uc} = \alpha p_{ua}p_{ub}p_{uc} + (1-\alpha )q_{ua}q_{ub}q_{uc}.
	\end{align*}
	
	Finally,  when the four nodes $u$, $a$, $b$ and $c$ forms a \underline{line graph} (Fig.~\ref{fig:line}) under general mixture model 
	\begin{gather*}
	1)~Y^|_{ua, ub} = \alpha  p_{ua}p_{ub} + (1- \alpha)  q_{ua}q_{ub},
	2)~Y^|_{ub, bc} = \alpha  p_{ub}p_{bc} + (1- \alpha)  q_{ub}q_{bc},\\
	3)~Z^|_{ua, ub, bc} = \alpha p_{ua}p_{ub}p_{bc} + (1-\alpha )q_{ua}q_{ub}q_{bc}.
	\end{gather*}
\end{claim}
The proof of the above claim is omitted as it follows closely the proofs of Claim~\ref{cl:trivialXab}, \ref{claim:eststar}, and \ref{claim:estline}.

\subsection{Star Graph}

We now present the following two lemmas which recover  the weights $p_{ui}$,and  $q_{ui}$ for all $ i\in \{a,b,c\}$ in the star graph (Fig.~\ref{fig:star}), and the general mixture parameter $\alpha$, respectively. 


\begin{lemma}[Weights of General Star Graph]\label{lem:stargen}
	Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, for the $star$ structure $(u,a,b,c)$ with $u$ as the central vertex the weight of any edge $(u,a)$  is given by:
	\begin{align*}
	p_{ua} &= X_{ua} + s_{ua}\sqrt{\tfrac{1-\alpha}{\alpha}} \sqrt{\frac{(Y_{ua,ub} - X_{ua}X_{ub})(Y_{ua,uc} - X_{ua}X_{uc})}{Y_{ub,uc} - X_{ub}X_{uc}}}\\ 
	q_{ua} &= X_{ua} - s_{ua} \sqrt{\tfrac{\alpha}{1-\alpha}} \sqrt{\frac{(Y_{ua,ub} - X_{ua}X_{ub})(Y_{ua,uc} - X_{ua}X_{uc})}{Y_{ub,uc} - X_{ub}X_{uc}}}
	\end{align*} 
	where $s_{ua} \in \{-1,1\}$ and $b,c \in N_1(u) \cap N_2(u)$ such that $b,c \ne a$, $b\neq c$.
\end{lemma}
\begin{proof}
	We notice that for $r \neq j \in \{a,b,c\}$
	\begin{align*}
	\left(Y_{ui, uj} - X_{ui}X_{uj}\right) &= \left(\alpha p_{ui}p_{uj} + (1-\alpha) q_{ui}q_{uj}\right) -\left(  \alpha p_{ui} + (1-\alpha) q_{ui}\right)\left( \alpha p_{uj} + (1-\alpha) q_{uj}\right) \\
	&=  \alpha(1-\alpha)(p_{ui} - q_{ui})(p_{uj} - q_{uj}).
	\end{align*}
	The rest of the proof follows the same steps as given in the proof of Lemma~\ref{lem:star} with the above modification.
\end{proof}


\begin{comment}
\begin{lemma}[$\alpha$  for General Star Graph]\label{lem:starAlpha}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, for the $star$ structure $(u,a,b,c)$ with $u$ as the central vertex, the general mixture parameter $\alpha$ is recovered as for $s_{\alpha} \in \{-1,+1\}$,
	\begin{align*}
	\alpha = \tfrac{1}{2}\left(1 + s_{\alpha} 
	\frac{
		\left(Z_{ua,ub,uc} 
		- \prod\limits_{ i\in \{a,b,c\}}X_{ui} 
		- \sum\limits_{ i, j, k\in \sigma(\{a,b,c\}) } X_{ui}\tilde{X}_{uj}\tilde{X}_{uk} \right)
	}
	{
		\sqrt{
			4 \left( \prod\limits_{ i\in \{a,b,c\}} \tilde{X}_{ui}\right)^2  
			+ \left(Z_{ua,ub,uc} 
			- \prod\limits_{ i\in \{a,b,c\}}X_{ui}
			- \sum\limits_{ i, j, k\in \sigma(\{a,b,c\}) } X_{ui}\tilde{X}_{uj}\tilde{X}_{uk} \right)^2
		}
	}\right)
	\end{align*}
	where for all $i, j, k \in \{a,b,c\}$, 
	$ \tilde{X}_{ui} = s_{ui}\sqrt{\frac{(Y_{ui,uj} - X_{ui}X_{uj})(Y_{ui,uk} - X_{ui}X_{uk})}{Y_{uj,uk} - X_{uj}X_{uk}}}.$
\end{lemma}
\begin{proof}
	We obtain $\alpha$ using the estimator $Z_{ui,uj,uk} = \alpha p_{ui}p_{uj}p_{uk} + (1-\alpha) q_{ui}q_{uj}q_{uk}$. 
	\begin{align*}
	& \alpha p_{ui}p_{uj}p_{uk} 
	= \alpha \prod_{i \in \{a,b,c\} }\left(X_{ui} + \tfrac{\sqrt{(1-\alpha)}}{\sqrt{\alpha}}\tilde{X}_{ui}\right)\\
	& = \alpha \prod_{i \in \{a, b, c\}}  X_{ui} 
	+  \sqrt{\alpha(1-\alpha)} \sum\limits_{(i,j,k) \in \sigma(\{a,b,c\})} X_{ui} X_{uj}\tilde{X}_{uk}\\
	&+ (1-\alpha) \sum\limits_{(i,j,k) \in \sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk} 
	+ \tfrac{(1-\alpha)^{3/2}}{\sqrt{\alpha}}\prod_{i \in \{a, b, c\}}  \tilde{X}_{ui}.
	\end{align*}
	Similarly, swapping the role of $\alpha$ and $(1-\alpha)$, and $\tilde{X}_{ui}$ and $- \tilde{X}_{ui}$ for all $i\in \{a,b,c\}$, we can easily obtain,
	\begin{align*}
	&(1-\alpha) q_{ui}q_{uk}q_{uk} \\
	&= (1-\alpha) \prod_{i \in \{a, b, c\}}  X_{ui} 
	-  \sqrt{\alpha(1-\alpha)} \sum\limits_{(i,j,k) \in \sigma(\{a,b,c\})} X_{ui} X_{uj}\tilde{X}_{uk}\\
	&+ \alpha \sum\limits_{(i,j,k) \in \sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk} 
	- \tfrac{\alpha^{3/2}}{\sqrt{(1-\alpha)}}\prod_{i \in \{a, b, c\}}  \tilde{X}_{ui}.
	\end{align*}
	
	Next taking the summation of the two terms we obtain,
	\begin{align}
	i)~&Z_{ui,uj,uk} \nonumber\\
	&=\prod_{i \in \{a, b, c\}}  X_{ui} 
	+ \sum\limits_{(i,j,k) \in \sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk} 
	+ \left(\tfrac{(1-\alpha)^{3/2}}{\sqrt{\alpha}}- \tfrac{\alpha^{3/2}}{\sqrt{(1-\alpha)}}\right) \prod_{i \in \{a, b, c\}}  \tilde{X}_{ui}.\label{eq:Z}\\
	%
	ii)~&\left(\prod_{i \in \{a, b, c\}}  \tilde{X}_{ui}\right) ((1-\alpha)^2 - \alpha^2) \nonumber\\
	&= \left(Z_{ui,uj,uk} - \prod_{i\in \{a,b,c\}} X_{ui} - \sum_{(i,j,k) \in\sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk}\right) \sqrt{\alpha(1-\alpha)} \nonumber\\
	%
	iii)~&\left(\prod_{i \in \{a, b, c\}}  \tilde{X}_{ui}\right)^2(1- 4\alpha + 4\alpha^2) \nonumber\\
	&= \left(Z_{ui,uj,uk} - \prod_{i\in \{a,b,c\}} X_{ui} - \sum_{(i,j,k) \in\sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk}\right)^2 \alpha(1-\alpha) \nonumber\\
	iv)~&(\alpha^2 - \alpha) 
	+ \tfrac{\left(\prod\limits_{i \in \{a, b, c\}}  \tilde{X}_{ui} \right)^2}
	{4 \left(\prod\limits_{i \in \{a, b, c\}}  \tilde{X}_{ui} \right)^2 + 
		\left(Z_{ui,uj,uk} - \prod\limits_{i\in \{a,b,c\}} X_{ui} 
		- \sum\limits_{(i,j,k) \in\sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk}\right)^2} 
	= 0 \nonumber\\
	%
	v)~&\alpha = \tfrac{1}{2}\left(1 \pm 
	\sqrt{
		\frac{
			\left(Z_{ui,uj,uk} - \prod\limits_{i\in \{a,b,c\}} X_{ui} 
			- \sum\limits_{(i,j,k) \in\sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk}\right)^2	
		}
		{
			4 \left(\prod\limits_{i \in \{a, b, c\}}  \tilde{X}_{ui} \right)^2  
			+ 
			\left(Z_{ui,uj,uk} - \prod\limits_{i\in \{a,b,c\}} X_{ui} 
			- \sum\limits_{(i,j,k) \in\sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk}\right)^2
		}
	}
	\right) \nonumber
	\end{align}
\end{proof}


\begin{lemma}[Sign Ambiguity Star Graph]\label{lem:starSign}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, for edges $(u,a), (u,b)$ for the $star$ structure $(u,a,b,c)$ with $u$ as the central vertex, the sign pattern $s_{ua}, s_{ub}$ satisfy the following relation.
	\[
	s_{ub}s_{ua} = \mathsf{sgn}(Y_{ua,ub} - X_{ua}X_{ub}).
	\]
	
	Furthermore, the sign pattern $s_{\alpha}$ is a function of  the sign pattern $s_{ub}$ (as mentioned in the proof below). The different choices of the sign pattern  $s_{ub}$ lead to a \emph{unique solution}, upto swapping of  $p_e$ and $q_e$ for all $e\in E$. 
	
\end{lemma}
\begin{proof}
	The proof of the first statement follows the same logic as the proof of Lemma~\ref{lem:signgen}, after noting that $\mathsf{sgn}(\alpha(1-\alpha)) = 1$ for $\alpha \in (0,1)$. 
	
	We now show that t$s_{\alpha}$ is not free and it is also dependent on $s_{ua}$.  Notice that from Eq.~\ref{eq:Z} we obtain, 
	$$\frac{2(1/2-\alpha)}{\sqrt{\alpha(1-\alpha)}} 
	= \frac{\left(
		Z_{ui,uj,uk} - \prod\limits_{i\in \{a,b,c\}} X_{ui} 
		- \sum\limits_{(i,j,k) \in\sigma(\{a,b,c\})} X_{ui} \tilde{X}_{uj}\tilde{X}_{uk}
		\right)}{\prod_{i\in \{a,b,c\}} \tilde{X}_{ui}}.$$
	
	This  fixes whether $\alpha > 1/2$  or $ \alpha< 1/2$, i.e. fixes the sign ambiguity, as a function of $s_{ua}$.  We also note $\alpha(s_{ua}) = (1- \alpha(-s_{ua}))$. Therefore, the choice of $s_{ua}$ simply swaps the two terms $\sqrt{\tfrac{1-\alpha(s_{ua})}{\alpha(s_{ua})}}s_{ua}$ and $\sqrt{\tfrac{\alpha(s_{ua})}{1-\alpha(s_{ua})}}(-s_{ua})$. Thus $s_{ua}$ swaps $p_{e}$ and $q_{e}$ for all $e\in E$.
\end{proof}
\end{comment}

\begin{lemma}[Sign Ambiguity Star Graph]\label{lem:starSign}
	Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, for edges $(u,a), (u,b)$ for the $star$ structure $(u,a,b,c)$ with $u$ as the central vertex, the sign pattern $s_{ua}, s_{ub}$ satisfy the following relation.
	\[
	s_{ub}s_{ua} = \mathsf{sgn}(Y_{ua,ub} - X_{ua}X_{ub}).
	\]
\end{lemma}
\begin{proof}
	The proof of the first statement follows the same logic as the proof of Lemma~\ref{lem:signgen}, after noting that $\mathsf{sgn}(\alpha(1-\alpha)) = 1$ for $\alpha \in (0,1)$. 
\end{proof}

\subsection{Line Graph}
We now present the recovery of parameters in the case of a line graph with knowledge of $\alpha$

\begin{lemma}[Weights of General Line Graph]\label{lem:linegen}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, the weights of the edges $(u,a)$, and $(u,b)$ for a $line$ graph $a-u-b-c$ can be learned in closed form (as given in the proof), as a function of\\
	(1) the mixture parameter $\alpha$,  \\
	(2) estimators $X_{ua}$, $X_{ub}$, $X_{bc}$, $Y^|_{ua,ub}$, $Y^|_{ub,bc}$, and $Z^|_{ua,ub,bc}$,\\ 
	(3) one variable $s_{ub} \in \{-1,+1\}$.
\end{lemma}
\begin{proof}
	We first note that we have access to the following three relations 
	\begin{align*}
	1)\quad&(Y^|_{ua,ub} - X_{ua}X_{ub}) = \alpha(1-\alpha) (p_{ua} - q_{ua})(p_{ub} - q_{ub})\\
	2)\quad&(Y^|_{ub,bc} - X_{ub}X_{bc}) = \alpha(1-\alpha) (p_{ub} - q_{ub})(p_{bc} - q_{bc})\\
	3)\quad&(Z^|_{ua, ub, bc} + X_{ua}X_{ub}X_{bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub})\\
	&= \alpha(1-\alpha)((1 - \alpha)p_{ub} + \alpha q_{ub})(p_{ua} - q_{ua})(p_{bc} - q_{bc}).
	\end{align*} 
	The first two inequalities follow similar to Lemma~\ref{lem:line}. We derive the final equality below.
	\begin{align*}
	&Z^|_{ua, ub, bc} + X_{ua}X_{ub}X_{bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}\\
	&= \alpha p_{ua}p_{ub}p_{bc} + (1- \alpha)q_{ua}q_{ub}q_{bc}\\
	&- (\alpha p_{ua} + (1 - \alpha)q_{ua})((\alpha p_{ub}p_{bc} + (1 - \alpha)q_{ub}q_{bc}) - (\alpha p_{bc} + (1 - \alpha)q_{bc})((\alpha p_{ua}p_{ub} + (1 - \alpha)q_{ua}q_{ub})\\
	& + (\alpha p_{ua} + (1 - \alpha)q_{ua})(\alpha p_{ub} + (1 - \alpha)q_{ub})(\alpha p_{bc} + (1 - \alpha)q_{bc})\\
	&=  \alpha (1 - \alpha)^2 p_{ua}p_{ub}p_{bc} + \alpha^2(1- \alpha)q_{ua}q_{ub}q_{bc}\\
	&- \alpha(1-\alpha)^2p_{ua}p_{ub}q_{bc}  + \alpha^2(1- \alpha)p_{ua}q_{ub}p_{bc} 
	- \alpha(1-\alpha)^2q_{ua}p_{ub}p_{bc}\\
	&- \alpha^2(1-\alpha)q_{ua}q_{ub}p_{bc} + \alpha(1-\alpha)^2q_{ua}p_{ub}q_{bc}  -\alpha^2(1-\alpha)p_{ua}q_{ub}q_{bc}\\
	&= \alpha(1-\alpha)((1 - \alpha)p_{ub} + \alpha q_{ub})(p_{ua} - q_{ua})(p_{bc} - q_{bc})
	\end{align*} 
	
	Therefore, we obtain the following quadratic equation in $p_{ub}$ and $q_{ub}$ (unlike the $\alpha = 1/2$ case it cannot be easily reduced to a linear equation),
	\[
	\frac{\alpha(1-\alpha)(p_{ub} - q_{ub})^2}{((1 - \alpha)p_{ub} + \alpha q_{ub})}= \frac{(Y^|_{ua,ub} - X_{ua}X_{ub})(Y^|_{ub,bc} - X_{ub}X_{bc})}{(Z^|_{ua, ub, bc} + X_{ua}X_{ub}X_{bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub})} := C_{ub}^|
	\]
	Note that $X_{ub} = \alpha p_{ub} + (1- \alpha)q_{ub}$, thus the above can be reduced to 
	\begin{align*}
	& \frac{\alpha(1-\alpha)(p_{ub}- X_{ub})^2/(1-\alpha)^2}{(p_{ub}(1- 2\alpha)+ \alpha X_{ub})/(1-\alpha)} = C_{ub}^|\\
	& p_{ub}^2 - 2\left(X_{ub}+ \tfrac{(1-2\alpha)}{2\alpha}C_{ub}^|\right)p_{ub} = C_{ub}^| X_{ub} - X^2_{ub}\\
	&p_{ub} = X_{ub} + \tfrac{(1-2\alpha)}{2\alpha} C_{ub}^| 
	+s_{ub}\sqrt{\left(\tfrac{(1-2\alpha)}{2\alpha} C_{ub}^| \right)^2 + \tfrac{1-\alpha}{\alpha}C_{ub}^| X_{ub} }\\
	& q_{ub} = X_{ub} - \tfrac{(1-2\alpha)}{2(1-\alpha)} C_{ub}^| 
	- s_{ub}\sqrt{\left(\tfrac{(1-2\alpha)}{2(1-\alpha)} C_{ub}^| \right)^2 + \tfrac{\alpha}{1-\alpha}C_{ub}^| X_{ub} }
	\end{align*}
	We substitute in the above two equations $\theta$ and $s_{\alpha}$ as defined below
	$$\alpha = \tfrac{1}{2}(1 - s_{\alpha}\sqrt{\theta}), 
	\qquad (1-\alpha) = \tfrac{1}{2}(1 + s_{\alpha}\sqrt{\theta}),
	\qquad (1-2\alpha) = s_{\alpha}\sqrt{\theta}.$$ 
	From the substitution we obtain,
	\begin{align*}
	&p_{ub} = X_{ub} +
	\tfrac{s_{\alpha}\sqrt{\theta}(1 + s_{\alpha}\sqrt{\theta})C^|_{ub}}{(1-\theta)}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{\theta C^|_{ub}}} \right)\\
	&q_{ub} = X_{ub} -
	\tfrac{s_{\alpha}\sqrt{\theta}(1 - s_{\alpha}\sqrt{\theta})C^|_{ub}}{(1-\theta)}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{ \theta C^|_{ub}}} \right)
	\end{align*}
	
	Next we use $p_{ub}$, and $q_{ub}$ to obtain $p_{ua}$, and $q_{ua}$. Specifically, we have
	\begin{align*}
	&\alpha(1-\alpha)(p_{ub} - q_{ub})(p_{ua} - q_{ua}) = (Y_{ua, ub}^| - X_{ua} X_{ub})\\
	&(p_{ua} - q_{ua})  = \frac{4(Y_{ua, ub}^| - X_{ua} X_{ub})}{ s_{\alpha} \sqrt{\theta}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{ \theta C^|_{ub}}} \right)}.
	\end{align*}
	
	
	Finally, we use the above relation to arrive at the required result.
	\begin{align*}
	&p_{ua} = X_{ua} +\frac{2(1+s_{\alpha}\sqrt{\theta}) (Y_{ua, ub}^| - X_{ua} X_{ub})}{ s_{\alpha} \sqrt{\theta}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{ \theta C^|_{ub}}} \right)}\\
	&q_{ua} = X_{ua} - \frac{2(1-s_{\alpha}\sqrt{\theta}) (Y_{ua, ub}^| - X_{ua} X_{ub})}{ s_{\alpha} \sqrt{\theta}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{ \theta C^|_{ub}}} \right)}
	\end{align*}
\end{proof}

\begin{comment}
We can not learn $\alpha$ along with the edge weights only from the line graph on $4$ nodes as there are $6$ independent equations and $7$ (including $\alpha$) unknowns. Therefore, we consider the line graph on $5$ nodes.

\begin{lemma}[$\alpha$ of General Line Graph]\label{lem:lineAlpha}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, the mixture parameter $\alpha$ for a line structure $a-u-b-c-d$ can be learned in a closed form (as given in the proof), where the coefficients are functions of\\ 
	(1) estimators $X_{ua}$, $X_{ub}$, $X_{bc}$, $X_{cd}$, $Y^|_{ua,ub}$, $Y^|_{ub,bc} = Y^|_{bu,bc}$, $Y^|_{bc,bd}$, $Z^|_{ua,ub,bc}$, $Z^|_{bu,bc,cd}$ \\
	(2) one variable $s_{\alpha} \in \{-1,+1\}$.
\end{lemma}
\begin{proof}
	We need to define the two following  quantities.
	$$
	C_{ub}^| = \frac{(Y^|_{ua,ub} - X_{ua}X_{ub})(Y^|_{ub,bc} - X_{ub}X_{bc})}{(Z^|_{ua, ub, bc} + X_{ua}X_{ub}X_{bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub})},
	$$
	$$
	C_{bc}^| = \frac{(Y^|_{bu,bc} - X_{bu}X_{bc})(Y^|_{bc,cd} - X_{bc}X_{cd})}{(Z^|_{bu, bc, cd} + X_{bu}X_{bc}X_{cd} - X_{bu}Y^|_{bc, cd} - X_{cd}Y^|_{bu,bc})}.
	$$
	Let us denote $\theta = (1-2\alpha)^2$ and let $s_{\alpha}\in\{-1,+1\}$ be such that  $ \alpha = \tfrac{1}{2}(1 - s_{\alpha}\sqrt{\theta})$.  
	
	We can obtain the estimate 
	$$(p_{ub} - q_{ub}) = \tfrac{2s_{\alpha}\sqrt{\theta} C^|_{ub}}{(1-\theta)}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{\theta C^|_{ub}}} \right)$$
	$$(p_{bc} - q_{bc}) = \tfrac{2s_{\alpha}\sqrt{\theta} C^|_{bc}}{(1-\theta)}\left( 1 + s_{\alpha} s_{bc} \sqrt{1+ \tfrac{(1-\theta)X_{bc}}{\theta C^|_{bc}}} \right).$$
	$$
	(Y^|_{ub,bc} - X_{ub}X_{bc}) 
	= \tfrac{\theta C^|_{ub} C^|_{bc}}{(1-\theta)}\left( 1 + s_{\alpha} s_{ub} \sqrt{1+ \tfrac{(1-\theta)X_{ub}}{\theta C^|_{ub}}} \right)\left( 1 + s_{\alpha} s_{bc} \sqrt{1+ \tfrac{(1-\theta)X_{bc}}{\theta C^|_{bc}}} \right)
	$$
	
	Let us also denote $\gamma = \tfrac{(1-\theta)}{\theta}$, $c_0 = \tfrac{Y^|_{ub,bc}}{X_{ub}X_{bc}} $,  $c_1 = \sqrt{\tfrac{C^|_{ub}}{X_{ub}}}$, and $c_2 = \sqrt{\tfrac{C^|_{bc}}{X_{bc}}}$. 
	After substitution the terms in the above equation we have the  following equation in $\gamma$.
	\begin{align}\label{eq:theta}
	&\left(c_0-1 \right) \gamma
	= c_1 c_2\left( c_1 +  s_{\alpha} s_{ub}\sqrt{c_1^2+ \gamma} \right)\left( c_2 +  s_{\alpha} s_{bc} \sqrt{c_2^2+ \gamma} \right)
	\end{align}
	
	As $\gamma \neq 0$, by assumption, there is a unique solution to the above equation for all possible values of $s_{\alpha}, s_{ub}, s_{bc} \in \{-1,+1\}$, which is given in closed form as
	\begin{align*}
	\gamma &= \frac{4 (c_0 -1) c_1^2 c_2^2 (c_0 - 1  + c_1^2) (c_0 - 1 + c_2^2)}{(c_0-1 - c_1 c_2)^2(c_0-1 +c_1 c_2)^2}\\
	&=  \frac{4 (Y^|_{ub,bc} - X_{ub}X_{bc})C^|_{ub} C^|_{bc} (Y^|_{ub,bc} - X_{ub}X_{bc} + C^|_{ub} X_{bc}) (Y^|_{ub,bc} - X_{ub}X_{bc} + C^|_{bc} X_{ub})}{( (Y^|_{ub,bc} - X_{ub}X_{bc})^2 - C^|_{ub} C^|_{bc} X_{ub}X_{bc} )^2}.
	\end{align*}
	This gives us the closed form expression for $\alpha = \tfrac{1}{2}(1 - s_{\alpha}\tfrac{1}{\sqrt{1+\gamma}})$.  
\end{proof}

\begin{lemma}[Sign Ambiguity Line graph on $5$ nodes]\label{lem:lineSign}
		Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, for a line structure $a-u-b-c-d$ the sign patterns  $s_{ub}$ and $s_{bc}$ satisfy the relation, $s_{ub} s_{bc} = \mathsf{sgn}(Y^|_{ub,bc} - X_{ub}X_{bc})$. 
	
	Furthermore, the sign pattern $s_{\alpha}$ is a function of  the sign pattern $s_{ub}$ (as mentioned in the proof below). The different choices of the sign pattern  $s_{ub}$ lead to a \emph{unique solution}, upto swapping of  $p_e$ and $q_e$ for all $e\in E$. 
\end{lemma}
\begin{proof}
	In proof of Lemma~\ref{lem:lineAlpha}, we use three sign quantities $s_{bc}$, $s_{ub}$, and $s_{\alpha}$. From the expression of $p_{ub}$ and $q_{ub}$ in Lemma~\ref{lem:linegen} we have ${\mathsf{sgn}(p_{ub} - q_{ub}) = s_{\alpha} s_{\alpha} s_{ub} = s_{ub}}$. Similarly, we obtain ${s_{bc} = \mathsf{sgn}(p_{bc} - q_{bc})}$. Therefore,  $s_{bc}s_{ub}  = \mathsf{sgn}(Y^|_{ub,bc} - X_{ub}X_{bc}).$ 
	
	
	We observe that $s_{\alpha}$ can be recovered as a function of $s_{ub}$
	\begin{align*}
	s_{\alpha}   =& 
	s_{ub} \times \mathsf{sgn}\left(\tfrac{\gamma (Y^|_{ub,bc} - X_{ub}X_{bc})}{C^|_{ub} C^|_{bc}} - 1 - s_{ub}s_{bc} \sqrt{1+ \gamma\tfrac{X_{ub}}{C^|_{ub}}}  \sqrt{1+ \gamma\tfrac{X_{bc}}{C^|_{bc}}}\right)\\
	&\times \mathsf{sgn}\left(\sqrt{1+ \gamma\tfrac{X_{ub}}{C^|_{ub}}} +  s_{ub}s_{bc} \sqrt{1+ \gamma\tfrac{X_{bc}}{C^|_{bc}}} \right).
	\end{align*}
	We  also observe that when $s_{\alpha}$ is changed,  the pairs 1) $\alpha$ and $(1-\alpha)$, 2) $p_{ub}$ and $q_{ub}$,  exchange values simultaneously. 
\end{proof}
\end{comment}

\begin{lemma}[Sign Ambiguity Line graph on $5$ nodes]\label{lem:lineSign}
	Under Conditions \ref{ass:necessary} and  \ref{ass:main}, in the setting of infinite samples, for a line structure $a-u-b-c-d$ the sign patterns  $s_{ub}$ and $s_{bc}$ satisfy the relation, $s_{ub} s_{bc} = \mathsf{sgn}(Y^|_{ub,bc} - X_{ub}X_{bc})$. 
\end{lemma}
\begin{proof}
	The proof is almost identical to the other sign ambiguity proofs.
\end{proof}

\subsection{Finite Sample Complexity}

We start by observing that the Claim~\ref{cl:Mu} still holds in the general case.
\begin{claim}\label{cl:epsilongeneral}
	If we can estimate $X_{ua}, Y^*_{ua,ub}, Y^|_{ua,ab}$ and $Z^|_{ua,ub,bc}$ within $\epsilon_1$, we can estimate $p_{ua}$  and $q_{ua}$ within precision 
	$\epsilon = \mathcal{O}\left( \epsilon_1 / \min(p_{min}, \Delta)^5 \min(\alpha, 1- \alpha)^4\right) $.
\end{claim}
\begin{proof}
	The proof proceeds in a very similar manner as Claim\ref{cl:epsilon2}. Following the derivations for $\hat{p}_{ua}$ and $\hat{q}_{ua}$ in the proof of Claim\ref{cl:epsilon2},  we can see that for the star primitive all the computation carry over with a scaling of $\tfrac{4}{\alpha(1-\alpha)}$ as we have 
	$Y^*_{ur,us} - X_{ur}X_{us} \geq \Delta^2 \alpha(1-\alpha)$ instead of $\Delta^2 /4$. 
	
	The line primitive presents with increased difficulty as the estimator is more complex. We first observe that $ \alpha(1-\alpha) \Delta^2 \leq C_{ub}^| \leq \max(\alpha, (1-\alpha))$. 
	We recall that 
	\begin{align*}
	&(Z^|_{ua, ub, bc} + X_{ua}X_{ub}X_{bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub}) \\
	&= \alpha(1-\alpha) ((1 - \alpha)p_{ub} + \alpha q_{ub})(p_{ua} - q_{ua})(p_{bc} - q_{bc})\\
	&\geq \min(\alpha, 1-\alpha)^2p_{min} \min(p_{min}, \Delta)^2/2,\\
	& (Y^|_{ua,ub} - X_{ua}X_{ub}) = \alpha(1-\alpha) (p_{ua} - q_{ua})(p_{ub} - q_{ub})
	\geq  \min(\alpha, 1-\alpha) \min(p_{min}, \Delta)^2/2.
	\end{align*}
	Let us assume the error in $(Z^|_{ua, ub, bc} + X_{ua}X_{ub}X_{bc} - X_{ua}Y^|_{ub, bc} - X_{bc}Y^|_{ua,ub})$ is bounded as $\epsilon_d$ and the error in $(Y^|_{ua,ub} - X_{ua}X_{ub}) (Y^|_{ub,bc} - X_{ub}X_{bc})$ is bounded as $\epsilon_n$. We have $\epsilon_n \leq 4\epsilon_1$ and $\epsilon_d \leq 3\epsilon_1$ as all the estimators are assumed to have error bounded by $\epsilon_1$. 
	
	
	Therefore, using  $|x/y - \hat{x}/\hat{y}| \leq x/y(\delta_x/x  +\delta_y/y)+ \mathcal{O}(\delta_x\delta_y)$,
	\begin{align*}
	| \hat{C}_{ub}^|  - C_{ub}^| | \leq \epsilon_c &:=  \mathcal{O}\left(\tfrac{\epsilon_n}{  \min(\alpha, 1-\alpha)^2  \min(p_{min}, \Delta)^4}
	+  \tfrac{\epsilon_d} { \min(\alpha, 1-\alpha)^2 p_{min} \min(p_{min}, \Delta)^2}  \right) \\
	&= \mathcal{O}(\epsilon_1/ \min(\alpha, 1-\alpha)^2  \min(p_{min}, \Delta)^4).
	\end{align*}
	
	Using the above bound in the expression of $p_{ua}$ we can obtain, 
	\begin{align*}
	&| \hat{p}_{ua} - p_{ua}| 
	%
	\leq | \hat{X}_{ua} - X_{ua}| + \tfrac{(1-2\alpha)}{2\alpha} |\hat{C}^|_{ua} - C^|_{ua}| + \dots\\ 
	&+ \big\lvert \sqrt{\left(\tfrac{(1-2\alpha)}{2\alpha} \hat{C}^|_{ua}\right)^2+\tfrac{(1-\alpha)}{\alpha} \hat{C}^|_{ua} \hat{X}_{ua}}
	-  \sqrt{\left(\tfrac{(1-2\alpha)}{2\alpha} C^|_{ua}\right)^2+\tfrac{(1-\alpha)}{\alpha} C^|_{ua} X_{ua}} \big\rvert\\
	%
	&\leq | \hat{X}_{ua} - X_{ua}| + \tfrac{(1-2\alpha)}{2\alpha} |\hat{C}^|_{ua} - C^|_{ua}| + \dots \\
	&+\frac{\left(\tfrac{(1-2\alpha)}{2\alpha}\right)^2 |\hat{C}^|_{ua} - C^|_{ua}| (\hat{C}^|_{ua}  + C^|_{ua}) + \tfrac{(1-\alpha)}{\alpha} | \hat{C}^|_{ua} \hat{X}_{ua} - C^|_{ua} X_{ua}|}
	{\sqrt{\left(\tfrac{(1-2\alpha)}{2\alpha} C^|_{ua}\right)^2+\tfrac{(1-\alpha)}{\alpha} C^|_{ua} X_{ua}} }\\
	%
	& \leq \epsilon_1 + \tfrac{(1-2\alpha)}{2\alpha} \epsilon_c + \tfrac{2}{(1-\alpha)\min(p_{min}, \Delta)} \left(2 \left(\tfrac{(1-2\alpha)}{2\alpha}\right)^2 \epsilon_c  + \tfrac{(1-\alpha)}{\alpha} (\epsilon_1 + \epsilon_c)\right) + o(\epsilon_1) + o(\epsilon_c)\\
	&\leq \mathcal{O}(\epsilon_1/\min(p_{min}, \Delta) \alpha (1-\alpha)) + \mathcal{O}( \epsilon_c/\min(p_{min}, \Delta) \alpha^2 (1-\alpha)) + o(\epsilon_1) + o(\epsilon_c)
	\end{align*}
	Therefore, using the estimate of $\epsilon_c$ we obtain, 
	$$| \hat{p}_{ua} - p_{ua}| \leq \mathcal{O}\left( \epsilon_1 / \min(p_{min}, \Delta)^5 \alpha \min(\alpha, 1- \alpha)^3\right).$$
	Switching $\alpha$ and $(1-\alpha)$ gives us the same bounds for $|\hat{q}_{ua} - q_{ua}|$. 
\end{proof}
In the above derivation we have used $\sqrt{\left(\tfrac{(1-2\alpha)}{2\alpha} C^|_{ua}\right)^2+\tfrac{(1-\alpha)}{\alpha} C^|_{ua} X_{ua}} \geq (1-\alpha)\min(p_{min}, \Delta) / 2$. We now derive the above inequality. 
\begin{align*}
&\lvert \sqrt{\left(\tfrac{(1-2\alpha)}{2\alpha} C^|_{ua}\right)^2+\tfrac{(1-\alpha)}{\alpha} C^|_{ua} X_{ua}} \rvert
= | p_{ua} - X_{ua} - \tfrac{(1-2\alpha)}{2\alpha} C^|_{ua}|\\
%
&= \lvert (1-\alpha) (p_{ua} - q_{ua}) - \tfrac{(1-2\alpha)(1-\alpha) (p_{ua} - q_{ua})^2 }{2 ((1-\alpha)p_{ua}+\alpha q_{ua})  }\rvert \\
&\geq \begin{cases*}
(1-\alpha) \min(p_{min}, \Delta), (\alpha \geq 1/2 \wedge p_{ua} \geq q_{ua}) \vee (\alpha < 1/2 \wedge p_{ua} < q_{ua})\\
(1-\alpha) \min(p_{min}, \Delta)|1 - \tfrac{(1-2\alpha)}{2(1-\alpha)}|, (\alpha < 1/2 \wedge p_{ua} \geq q_{ua}) \\
(1-\alpha) \min(p_{min}, \Delta) |1 - \tfrac{(2\alpha-1)}{2\alpha}|, (\alpha \geq 1/2 \wedge p_{ua} < q_{ua}), 
\end{cases*}
\end{align*} 



Finally, using union bound on all the estimators involved accross all possible edges, we can obtain the error bound in the following Theorem~\ref{thm:mainexistgen}. 
\begin{theorem}\label{thm:mainexistgen}
	Suppose Condition \ref{ass:necessary} and \ref{ass:main} are true, there exists an algorithm that runs on epidemic cascades over a mixture of two undirected, weighted graphs $G_1 = (V, E_1)$ and $G_2 = (V, E_2)$, and recovers the edge weights corresponding to each graph up to precision $\epsilon$ in time $O(N^2)$ and sample complexity $O\left(\frac{N\log N}{\epsilon^2\Delta^4}\right)$ for $\alpha = 1/2$ and 
	$O\left(\frac{N\log N}{\epsilon^2\Delta^{10} \min(\alpha, 1-\alpha)^8 }\right)$ 
	for general $\alpha\in (0,1), \alpha \neq 1/2$, 
	where $N = |V|$.
\end{theorem}

